Exploring Chain-of-Thought Style Prompting for Text-to-SQL

In-context learning with large language models (LLMs) has recently caught increasing attention due to its superior few-shot performance on various tasks. However, its performance on text-to-SQL parsing still has much room for improvement. In this paper, we hypothesize that a crucial aspect of LLMs to improve for text-to-SQL parsing is their multi-step reasoning ability. Thus, we systematically study how to enhance LLMs' reasoning ability through chain of thought (CoT) style prompting, including the original chain-of-thought prompting (Wei et al., 2022b) and least-to-most prompting (Zhou et al., 2023). Our experiments demonstrate that iterative prompting as in Zhou et al. (2023) may be unnecessary for text-to-SQL parsing, and using detailed reasoning steps tends to have more error propagation issues. Based on these findings, we propose a new CoT-style prompting method for text-to-SQL parsing. It brings 5.2 and 6.5 point absolute gains on the Spider development set and the Spider Realistic set, respectively, compared to the standard prompting method without reasoning steps; 2.4 and 1.5 point absolute gains, compared to the least-to-most prompting method.

==> app_example/api_least_to_most.tex <==
% \noindent \textbf{\LTM + API Docs Prompting (Problem Reduction)} 

% \noindent An example prompt under least-to-most + API docs prompting (problem reduction) for 1-shot on Spider. \\

% An example prompt under standard prompting for 4-shot on Spider

\noindent \#\#\# SQLite SQL tables, with their properties:
\\
\# class (class\_code, crs\_code, class\_section, class\_time, class\_room, prof\_num)
\\
\# course (crs\_code, dept\_code, crs\_description, crs\_credit)
\\
\# department (dept\_code, dept\_name, school\_code, emp\_num, dept\_address, dept\_extension)
\\
\# employee (emp\_num, emp\_lname, emp\_fname, emp\_initial, emp\_jobcode, emp\_hiredate, emp\_dob)
\\
\# enroll (class\_code, stu\_num, enroll\_grade)
\\
\# professor (emp\_num, dept\_code, prof\_office, prof\_extension, prof\_high\_degree)
\\
\# student (stu\_num, stu\_lname, stu\_fname, stu\_init, stu\_dob, stu\_hrs, stu\_class, stu\_gpa, stu\_transfer, dept\_code, stu\_phone, prof\_num)
\\
\# 
To answer the question “Find the first names and offices of all instructors who have taught some course and the course description and the department name.”, we need to know: “Find the first names and offices of all instructors.”, “Find the first names and offices of all instructors who have taught some course.”, “Find the first names and offices of all instructors who have taught some course and the course description.”.
\\
\\
% \#\#\# SQLite SQL tables, with their properties:
% \\
% \# ref\_characteristic\_types (characteristic\_type\_code, characteristic\_type\_description)
% \\
% \# ref\_colors (color\_code, color\_description)
% \\
% \# ref\_product\_categories (product\_category\_code, product\_category\_description, unit\_of\_measure)
% \\
% \# characteristics (characteristic\_id, characteristic\_type\_code, characteristic\_data\_type, characteristic\_name, other\_characteristic\_details)
% \\
% \# products (product\_id, color\_code, product\_category\_code, product\_name, typical\_buying\_price, typical\_selling\_price, product\_description, other\_product\_details)
% \\
% \# product\_characteristics (product\_id, characteristic\_id, product\_characteristic\_value)
% \\
% \# 
% To answer the question “Find the number of the products that have their color described as "red" and have a characteristic named "slow".”, we need to know: “Find the number of the products that have their color.”, “Find the number of the products that have their color described as "red".”, “Find the number of the products that have their color described as "red" and have a characteristic.”.
% \\
% \\
% \#\#\# SQLite SQL tables, with their properties:
% \\
% \# station (station\_id, name, annual\_entry\_exit, annual\_interchanges, total\_passengers, location, main\_services, number\_of\_platforms)
% \\
% \# train (train\_id, name, time, service)
% \\
% \# train\_station (train\_id, station\_id)
% \\
% \# 
% To answer the question “Show all train names and times in stations in London in descending order by train time.”, we need to know: “Show all train names and times.”, “Show all train names and times in stations.”, “Show all train names and times in stations in London.”.
% \\
% \\
% \#\#\# SQLite SQL tables, with their properties:
% \\
% \# person (name, age, city, gender, job)
% \\
% \# personfriend (name, friend, year)
% \\
% \# 
% To answer the question “What is the age of the friend of Zach with longest year relationship?”, we need to know: “What is the age of the friend?”, “What is the age of the friend of Zach?”.
% \\
% \\
\#\#\# SQLite SQL tables, with their properties:
\\
\# stadium (stadium\_id, location, name, capacity, highest, lowest, average)
\\
\# singer (singer\_id, name, country, song\_name, song\_release\_year, age, is\_male)
\\
\# concert (concert\_id, concert\_name, theme, stadium\_id, year)
\\
\# singer\_in\_concert (concert\_id, singer\_id)
\\
\# 
To answer the question “How many singers do we have?”, we need to know: \\
\\

\noindent \textbf{\LTM + API Docs Prompting (Problem Solving)} 

An example prompt under least-to-most + API docs prompting (problem solving) for 1-shot on Spider. \\

% An example prompt under standard prompting for 4-shot on Spider


\noindent \#\#\# SQLite SQL tables, with their properties:
\\\# class (class\_code, crs\_code, class\_section, class\_time, class\_room, prof\_num)
\\\# course (crs\_code, dept\_code, crs\_description, crs\_credit)
\\\# department (dept\_code, dept\_name, school\_code, emp\_num, dept\_address, dept\_extension)
\\\# employee (emp\_num, emp\_lname, emp\_fname, emp\_initial, emp\_jobcode, emp\_hiredate, emp\_dob)
\\\# enroll (class\_code, stu\_num, enroll\_grade)
\\\# professor (emp\_num, dept\_code, prof\_office, prof\_extension, prof\_high\_degree)
\\\# student (stu\_num, stu\_lname, stu\_fname, stu\_init, stu\_dob, stu\_hrs, stu\_class, stu\_gpa, stu\_transfer, dept\_code, stu\_phone, prof\_num)
\\\# 
\\ Q: Find the first names and offices of all instructors.
\\ A: SELECT T1.emp\_fname ,  T2.prof\_office FROM employee AS T1 JOIN professor AS T2 ON T1.emp\_num  =  T2.emp\_num
\\
\\Q: Find the first names and offices of all instructors who have taught some course.
\\A: SELECT T2.emp\_fname ,  T4.prof\_office FROM CLASS AS T1 JOIN employee AS T2 ON T1.prof\_num  =  T2.emp\_num JOIN course AS T3 ON T1.crs\_code  =  T3.crs\_code JOIN professor AS T4 ON T2.emp\_num  =  T4.emp\_num 
\\
\\Q: Find the first names and offices of all instructors who have taught some course and the course description.
\\A: SELECT T2.emp\_fname ,  T4.prof\_office ,  T3.crs\_description FROM CLASS AS T1 JOIN employee AS T2 ON T1.prof\_num  =  T2.emp\_num JOIN course AS T3 ON T1.crs\_code  =  T3.crs\_code JOIN professor AS T4 ON T2.emp\_num  =  T4.emp\_num
\\
\\Q: Find the first names and offices of all instructors who have taught some course and the course description and the department name.
\\A: SELECT T2.emp\_fname ,  T4.prof\_office ,  T3.crs\_description ,  T5.dept\_name FROM CLASS AS T1 JOIN employee AS T2 ON T1.prof\_num  =  T2.emp\_num JOIN course AS T3 ON T1.crs\_code  =  T3.crs\_code JOIN professor AS T4 ON T2.emp\_num  =  T4.emp\_num JOIN department AS T5 ON T4.dept\_code  =  T5.dept\_code
\\
\\
% \#\#\# SQLite SQL tables, with their properties:
% \\\# ref\_characteristic\_types (characteristic\_type\_code, characteristic\_type\_description)
% \\\# ref\_colors (color\_code, color\_description)
% \\\# ref\_product\_categories (product\_category\_code, product\_category\_description, unit\_of\_measure)
% \\\# characteristics (characteristic\_id, characteristic\_type\_code, characteristic\_data\_type, characteristic\_name, other\_characteristic\_details)
% \\\# products (product\_id, color\_code, product\_category\_code, product\_name, typical\_buying\_price, typical\_selling\_price, product\_description, other\_product\_details)
% \\\# product\_characteristics (product\_id, characteristic\_id, product\_characteristic\_value)
% \\\# 
% \\Q: Find the number of the products that have their color.
% \\A: SELECT count(*) FROM products AS t1
% \\
% \\Q: Find the number of the products that have their color described as "red".
% \\A: SELECT count(*) FROM products AS t1 JOIN ref\_colors AS t2 ON t1.color\_code  =  t2.color\_code WHERE t2.color\_description  =  "red"
% \\
% \\Q: Find the number of the products that have their color described as "red" and have a characteristic.
% \\A: SELECT count(*) FROM products AS t1 JOIN product\_characteristics AS t2 ON t1.product\_id  =  t2.product\_id JOIN ref\_colors AS t3 ON t1.color\_code  =  t3.color\_code WHERE t3.color\_description  =  "red"
% \\
% \\
% Q: Find the number of the products that have their color described as "red" and have a characteristic named "slow".
% \\A: SELECT count(*) FROM products AS t1 JOIN product\_characteristics AS t2 ON t1.product\_id  =  t2.product\_id JOIN CHARACTERISTICS AS t3 ON t2.characteristic\_id  =  t3.characteristic\_id JOIN ref\_colors AS t4 ON t1.color\_code  =  t4.color\_code WHERE t4.color\_description  =  "red" AND t3.characteristic\_name  =  "slow"
% \\
% \\
% \#\#\# SQLite SQL tables, with their properties:
% \\\# station (station\_id, name, annual\_entry\_exit, annual\_interchanges, total\_passengers, location, main\_services, number\_of\_platforms)
% \\\# train (train\_id, name, time, service)
% \\\# train\_station (train\_id, station\_id)
% \\\# 
% \\Q: Show all train names and times.
% \\A: SELECT T1.name ,  T1.time FROM train AS T1
% \\
% \\Q: Show all train names and times in stations.
% \\A: SELECT T2.name ,  T2.time FROM train\_station AS T1 JOIN train AS T2 ON T2.train\_id  =  T1.train\_id
% \\
% \\Q: Show all train names and times in stations in London.
% \\A: SELECT T3.name ,  T3.time FROM train\_station AS T1 JOIN station AS T2 ON T1.station\_id  =  T2.station\_id JOIN train AS T3 ON T3.train\_id  =  T1.train\_id WHERE T2.location  =  'London'
% \\
% \\Q: Show all train names and times in stations in London in descending order by train time.
% \\A: SELECT T3.name ,  T3.time FROM train\_station AS T1 JOIN station AS T2 ON T1.station\_id  =  T2.station\_id JOIN train AS T3 ON T3.train\_id  =  T1.train\_id WHERE T2.location  =  'London' ORDER BY T3.time DESC
% \\
% \\
% \#\#\# SQLite SQL tables, with their properties:
% \\\# person (name, age, city, gender, job)
% \\\# personfriend (name, friend, year)
% \\\# 
% \\Q: What is the age of the friend?
% \\A: SELECT T1.age FROM Person AS T1
% \\
% \\Q: What is the age of the friend of Zach?
% \\A: SELECT T1.age FROM Person AS T1 JOIN PersonFriend AS T2 ON T1.name  =  T2.friend WHERE T2.name =  'Zach'
% \\
% \\Q: What is the age of the friend of Zach with longest year relationship?
% \\A: SELECT T1.age FROM Person AS T1 JOIN PersonFriend AS T2 ON T1.name  =  T2.friend WHERE T2.name =  'Zach' AND T2.year  =  (SELECT max(t3.YEAR) FROM PersonFriend as t3 WHERE t3.name =  'Zach')
% \\
% \\
\#\#\# SQLite SQL tables, with their properties:
\\\# stadium (stadium\_id, location, name, capacity, highest, lowest, average)
\\\# singer (singer\_id, name, country, song\_name, song\_release\_year, age, is\_male)
\\\# concert (concert\_id, concert\_name, theme, stadium\_id, year)
\\\# singer\_in\_concert (concert\_id, singer\_id)
\\\# 
\\Q: How many singers?\\

==> app_example/app_numofexps.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{lcccc}
\toprule
& 0 & 1 & 4 & 8 \\ \midrule 
standard & 59.6 & 62.2 & 58.3 & 58.7      \\ \midrule 
least-to-most &-  & 63.7 & 63.0 & 63.3  \\ \midrule 
QDecomp  &- & 63.6 & 65.5 & 66.5 \\ \midrule 
+ interCOL  &-  & 66.4 & 67.3 & 68.8 \\ \midrule 
\end{tabular}
\caption{Test-suite accuracy with varying numbers of support examples, where the exemplars from G3 are used.}
\vspace{-10pt}
\label{tab:app_number_of_examples}
\end{table}

 % \hs{do you still need both Table 11 and 12?}

==> app_example/app_promptdesign.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{lcccc}
\toprule 
& API docs & Create Table + Select 3 \\ \midrule 
standard & 58.3 & 60.6 \\ \midrule 
least-to-most & 63.0 & 65.6 \\ \midrule
QDecomp & 65.5 & 66.9  \\ \midrule 
+ interCOL & 67.3 & 69.8  \\ \midrule 
\end{tabular}
\caption{The impact of different prompts design of providing schema information on test-site accuracy on the Spider, where the number of in-context exemplars is set to 4, where the exemplars from the G3 are used}
% \vspace{-10pt}
\label{tb:app_g3_impactofschemaprompt}
\end{table}

==> app_example/ctb_chain_of_thought.tex <==
% \noindent \textbf{Chain-of-thought + create table + select 3 prompting} 

% \noindent An example taken from the chain-of-thought promptings for 2-shot on the Spider dataset. \\



==> app_example/ctb_least_to_most.tex <==
\noindent \textbf{\LTM + Create Table + Select 3 prompting (Problem Reduction)} 

\noindent An example prompt under least-to-most + Create Table + Select 3 prompting (problem reduction) for 1-shot on Spider. \\

% An example prompt under standard prompting for 4-shot on Spider
% 


\noindent CREATE TABLE Customers (\\
customer\_id INTEGER PRIMARY KEY,\\
customer\_name VARCHAR(80),\\
customer\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Customers  LIMIT 3;\\
customer\_id customer\_name customer\_details \\
          1      Savannah            rerum \\
          2        George              est \\
          3       Alberto         deleniti \\
*/\\
\\
CREATE TABLE Invoices (\\
invoice\_number INTEGER PRIMARY KEY,\\
invoice\_date DATETIME,\\
invoice\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Invoices  LIMIT 3;\\
invoice\_number        invoice\_date invoice\_details \\
             1 1989-09-03 16:03:05           vitae \\
             2 1989-12-11 16:40:57          magnam \\
             3 1995-10-07 14:13:05              et \\
*/\\
\\
CREATE TABLE Orders (\\
order\_id INTEGER PRIMARY KEY,\\
customer\_id INTEGER NOT NULL,\\
order\_status VARCHAR(10) NOT NULL,\\
date\_order\_placed DATETIME NOT NULL,\\
order\_details VARCHAR(255),\\
FOREIGN KEY (customer\_id ) REFERENCES Customers(customer\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Orders  LIMIT 3;\\
order\_id customer\_id order\_status   date\_order\_placed order\_details \\
       1           2      Shipped 2009-02-21 15:26:19          None \\
       2          11      Shipped 1974-06-24 22:10:26          None \\
       3           4      Shipped 1982-12-29 21:10:11          None \\
*/\\
\\
CREATE TABLE Products (\\
product\_id INTEGER PRIMARY KEY,\\
product\_name VARCHAR(80),\\
product\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Products  LIMIT 3;\\
product\_id product\_name product\_details \\
         1         food            None \\
         2         book            None \\
         3         food            None \\
*/\\
\\
CREATE TABLE Order\_Items (\\
order\_item\_id INTEGER PRIMARY KEY,\\
product\_id INTEGER NOT NULL,\\
order\_id INTEGER NOT NULL,\\
order\_item\_status VARCHAR(10) NOT NULL,\\
order\_item\_details VARCHAR(255),\\
FOREIGN KEY (order\_id ) REFERENCES Orders(order\_id ),\\
FOREIGN KEY (product\_id ) REFERENCES Products(product\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Order\_Items  LIMIT 3;\\
order\_item\_id product\_id order\_id order\_item\_status order\_item\_details \\
            1          4        6            Finish               None \\
            2         15        6            Finish               None \\
            3         12       15            Finish               None \\
*/\\
\\
CREATE TABLE Shipments (\\
shipment\_id INTEGER PRIMARY KEY,\\
order\_id INTEGER NOT NULL,\\
invoice\_number INTEGER NOT NULL,\\
shipment\_tracking\_number VARCHAR(80),\\
shipment\_date DATETIME,\\
other\_shipment\_details VARCHAR(255),\\
FOREIGN KEY (order\_id ) REFERENCES Orders(order\_id ),\\
FOREIGN KEY (invoice\_number ) REFERENCES Invoices(invoice\_number )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Shipments  LIMIT 3;\\
shipment\_id order\_id invoice\_number shipment\_tracking\_number       shipment\_date other\_shipment\_details \\
          1        5             13                     3452 1983-08-13 22:34:11                   None \\
          2        7              2                     0114 1977-11-10 12:11:25                   None \\
          3       10              5                      478 2006-01-17 03:08:05                   None \\
*/\\
\\
CREATE TABLE Shipment\_Items (\\
shipment\_id INTEGER NOT NULL,\\
order\_item\_id INTEGER NOT NULL,\\
FOREIGN KEY (order\_item\_id ) REFERENCES Order\_Items(order\_item\_id ),\\
FOREIGN KEY (shipment\_id ) REFERENCES Shipments(shipment\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Shipment\_Items  LIMIT 3;\\
shipment\_id order\_item\_id \\
         11            12 \\
         10            15 \\
         10            12 \\
*/\\
\\
\\
To answer the question “What are the names of the customers who have made two or less orders?”, we need to know: “What are the names of the customers?”, “What are the names of the customers who have made orders?”. 
\\
% \\
% \\CREATE TABLE grapes (\\
% ID INTEGER PRIMARY KEY,\\
% Grape TEXT UNIQUE,\\
% Color TEXT\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM grapes  LIMIT 3;\\
% ID               Grape Color \\
%  1             Barbera   Red \\
%  2      Cabernet Franc   Red \\
%  3 Cabernet Sauvingnon   Red \\
%  */\\
% \\
% CREATE TABLE appellations (\\
% No INTEGER PRIMARY KEY,\\
% Appelation TEXT UNIQUE,\\
% County TEXT,\\
% State TEXT,\\
% Area TEXT,\\
% isAVA TEXT\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM appellations  LIMIT 3;\\
% No                       Appelation County      State             Area isAVA \\
%  1                 Alexander Valley Sonoma California      North Coast   Yes \\
%  2                    Amador County Amador California Sierra Foothills    No \\
%  3 Amador-Mendocino-Sonoma Counties    N/A California              N/A    No \\
%  */\\
% \\
% CREATE TABLE wine (\\
% No INTEGER,\\
% Grape TEXT,\\
% Winery TEXT,\\
% Appelation TEXT,\\
% State TEXT,\\
% Name TEXT,\\
% Year INTEGER,\\
% Price INTEGER,\\
% Score INTEGER,\\
% Cases INTEGER,\\
% Drink TEXT,\\
% FOREIGN KEY (Grape) REFERENCES grapes(Grape),\\
% FOREIGN KEY (Appelation) REFERENCES appellations(Appelation)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM wine  LIMIT 3;\\
% No     Grape           Winery  Appelation      State               Name Year Price Score Cases Drink \\
%  1 Zinfandel     Robert Biale  St. Helena California Old Kraft Vineyard 2008    44    93   275   now \\
%  2 Zinfandel Chiarello Family Napa Valley California              Giana 2008    35    93   480   now \\
%  3 Zinfandel     Robert Biale Napa Valley California      Black Chicken 2008    40    91  2700  2012 \\
%  */\\
% \\
% \\
% To answer the question “How many wines are produced at Robert Biale winery?”, we need to know: .
% \\
% \\
% \\
% CREATE TABLE Activity (\\
% actid INTEGER PRIMARY KEY,\\
% activity\_name varchar(25)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Activity  LIMIT 3;\\
% actid     activity\_name \\
%   770 Mountain Climbing \\
%   771          Canoeing \\
%   772          Kayaking \\
%   */\\
% \\
% CREATE TABLE Participates\_in (\\
% stuid INTEGER,\\
% actid INTEGER,\\
% FOREIGN KEY(stuid) REFERENCES Student(StuID),\\
% FOREIGN KEY(actid) REFERENCES Activity(actid)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Participates\_in  LIMIT 3;\\
% stuid actid \\
%  1001   770 \\
%  1001   771 \\
%  1001   777 \\
%  */\\
% \\
% CREATE TABLE Faculty\_Participates\_in (\\
% FacID INTEGER,\\
% actid INTEGER,\\
% FOREIGN KEY(FacID) REFERENCES Faculty(FacID),\\
% FOREIGN KEY(actid) REFERENCES Activity(actid)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Faculty\_Participates\_in  LIMIT 3;\\
% FacID actid \\
%  1082   784 \\
%  1082   785 \\
%  1082   790 \\
%  */\\
% \\
% CREATE TABLE Student (\\
% StuID        INTEGER PRIMARY KEY,\\
% LName        VARCHAR(12),\\
% Fname        VARCHAR(12),\\
% Age      INTEGER,\\
% Sex      VARCHAR(1),\\
% Major        INTEGER,\\
% Advisor      INTEGER,\\
% city\_code    VARCHAR(3)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Student  LIMIT 3;\\
% StuID LName  Fname Age Sex Major Advisor city\_code \\
%  1001 Smith  Linda  18   F   600    1121       BAL \\
%  1002   Kim  Tracy  19   F   600    7712       HKG \\
%  1003 Jones Shiela  21   F   600    7792       WAS \\
%  */\\
% \\
% CREATE TABLE Faculty (\\
% FacID          INTEGER PRIMARY KEY,\\
% Lname   VARCHAR(15),\\
% Fname   VARCHAR(15),\\
% Rank    VARCHAR(15),\\
% Sex   VARCHAR(1),\\
% Phone   INTEGER,\\
% Room    VARCHAR(5),\\
% Building    VARCHAR(13)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Faculty  LIMIT 3;\\
% FacID    Lname   Fname       Rank Sex Phone Room Building \\
%  1082 Giuliano    Mark Instructor   M  2424  224      NEB \\
%  1121 Goodrich Michael  Professor   M  3593  219      NEB \\
%  1148   Masson  Gerald  Professor   M  3402 224B      NEB \\
%  */\\
% \\
% \\
% To answer the question “Which rank has the smallest number of faculty members?”, we need to know: .\\
\\
\\
CREATE TABLE stadium (\\
Stadium\_ID int,\\
Location text,\\
Name text,\\
Capacity int,\\
Highest int,\\
Lowest int,\\
Average int,\\
PRIMARY KEY (Stadium\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM stadium  LIMIT 3;\\
Stadium\_ID     Location            Name Capacity Highest Lowest Average \\
         1 Raith Rovers    Stark's Park    10104    4812   1294    2106 \\
         2   Ayr United   Somerset Park    11998    2363   1057    1477 \\
         3    East Fife Bayview Stadium     2000    1980    533     864 \\
         */\\
\\
CREATE TABLE singer (\\
Singer\_ID int,\\
Name text,\\
Country text,\\
Song\_Name text,\\
Song\_release\_year text,\\
Age int,\\
Is\_male bool,\\
PRIMARY KEY (Singer\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM singer  LIMIT 3;\\
Singer\_ID         Name       Country Song\_Name Song\_release\_year Age Is\_male \\
        1    Joe Sharp   Netherlands       You              1992  52       F \\
        2    Timbaland United States Dangerous              2008  32       T \\
        3 Justin Brown        France    Hey Oh              2013  29       T \\
        */\\
\\
CREATE TABLE concert (\\
concert\_ID int,\\
concert\_Name text,\\
Theme text,\\
Stadium\_ID text,\\
Year text,\\
PRIMARY KEY (concert\_ID),\\
FOREIGN KEY (Stadium\_ID) REFERENCES stadium(Stadium\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM concert  LIMIT 3;\\
concert\_ID   concert\_Name         Theme Stadium\_ID Year \\
         1      Auditions   Free choice          1 2014 \\
         2 Super bootcamp Free choice 2          2 2014 \\
         3    Home Visits Bleeding Love          2 2015 \\
         */\\
\\
CREATE TABLE singer\_in\_concert (\\
concert\_ID int,\\
Singer\_ID text,\\
PRIMARY KEY (concert\_ID,Singer\_ID),\\
FOREIGN KEY (concert\_ID) REFERENCES concert(concert\_ID),\\
FOREIGN KEY (Singer\_ID) REFERENCES singer(Singer\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM singer\_in\_concert  LIMIT 3;\\
concert\_ID Singer\_ID \\
         1         2 \\
         1         3 \\
         1         5 \\
         */\\
\\
\\
To answer the question “How many singers do we have?”, we need to know: \\
\\
\noindent \textbf{\LTM + Create Table + Select 3 prompting (Problem Solving)}

\noindent An example prompt under least-to-most + Create Table + Select 3 prompting (problem solving) for 1-shot on Spider. \\


% \noindent An example prompt under \LTM + Create Table + Select 3 prompting (decomposition) for 1-shot on Spider. 



\noindent CREATE TABLE Customers (\\
customer\_id INTEGER PRIMARY KEY,\\
customer\_name VARCHAR(80),\\
customer\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Customers  LIMIT 3;\\
customer\_id customer\_name customer\_details \\
          1      Savannah            rerum \\
          2        George              est \\
          3       Alberto         deleniti \\
*/\\
\\
CREATE TABLE Invoices (\\
invoice\_number INTEGER PRIMARY KEY,\\
invoice\_date DATETIME,\\
invoice\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Invoices  LIMIT 3;\\
invoice\_number        invoice\_date invoice\_details \\
             1 1989-09-03 16:03:05           vitae \\
             2 1989-12-11 16:40:57          magnam \\
             3 1995-10-07 14:13:05              et \\
*/\\
\\
CREATE TABLE Orders (\\
order\_id INTEGER PRIMARY KEY,\\
customer\_id INTEGER NOT NULL,\\
order\_status VARCHAR(10) NOT NULL,\\
date\_order\_placed DATETIME NOT NULL,\\
order\_details VARCHAR(255),\\
FOREIGN KEY (customer\_id ) REFERENCES Customers(customer\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Orders  LIMIT 3;\\
order\_id customer\_id order\_status   date\_order\_placed order\_details \\
       1           2      Shipped 2009-02-21 15:26:19          None \\
       2          11      Shipped 1974-06-24 22:10:26          None \\
       3           4      Shipped 1982-12-29 21:10:11          None \\
*/\\
\\
CREATE TABLE Products (\\
product\_id INTEGER PRIMARY KEY,\\
product\_name VARCHAR(80),\\
product\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Products  LIMIT 3;\\
product\_id product\_name product\_details \\
         1         food            None \\
         2         book            None \\
         3         food            None \\
*/\\
\\
CREATE TABLE Order\_Items (\\
order\_item\_id INTEGER PRIMARY KEY,\\
product\_id INTEGER NOT NULL,\\
order\_id INTEGER NOT NULL,\\
order\_item\_status VARCHAR(10) NOT NULL,\\
order\_item\_details VARCHAR(255),\\
FOREIGN KEY (order\_id ) REFERENCES Orders(order\_id ),\\
FOREIGN KEY (product\_id ) REFERENCES Products(product\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Order\_Items  LIMIT 3;\\
order\_item\_id product\_id order\_id order\_item\_status order\_item\_details \\
            1          4        6            Finish               None \\
            2         15        6            Finish               None \\
            3         12       15            Finish               None \\
*/\\
\\
CREATE TABLE Shipments (\\
shipment\_id INTEGER PRIMARY KEY,\\
order\_id INTEGER NOT NULL,\\
invoice\_number INTEGER NOT NULL,\\
shipment\_tracking\_number VARCHAR(80),\\
shipment\_date DATETIME,\\
other\_shipment\_details VARCHAR(255),\\
FOREIGN KEY (order\_id ) REFERENCES Orders(order\_id ),\\
FOREIGN KEY (invoice\_number ) REFERENCES Invoices(invoice\_number )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Shipments  LIMIT 3;\\
shipment\_id order\_id invoice\_number shipment\_tracking\_number       shipment\_date other\_shipment\_details \\
          1        5             13                     3452 1983-08-13 22:34:11                   None \\
          2        7              2                     0114 1977-11-10 12:11:25                   None \\
          3       10              5                      478 2006-01-17 03:08:05                   None \\
*/\\
\\
CREATE TABLE Shipment\_Items (\\
shipment\_id INTEGER NOT NULL,\\
order\_item\_id INTEGER NOT NULL,\\
FOREIGN KEY (order\_item\_id ) REFERENCES Order\_Items(order\_item\_id ),\\
FOREIGN KEY (shipment\_id ) REFERENCES Shipments(shipment\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Shipment\_Items  LIMIT 3;\\
shipment\_id order\_item\_id \\
         11            12 \\
         10            15 \\
         10            12 \\
*/\\
\\
Q: What are the names of the customers?\\
A: SELECT customer\_name FROM customers\\
\\
Q: What are the names of the customers who have made orders?\\
A: SELECT T1.customer\_name FROM customers AS T1 JOIN orders AS T2 ON T1.customer\_id  =  T2.customer\_id\\
\\
Q: What are the names of the customers who have made two or less orders?\\
A: SELECT T1.customer\_name FROM customers AS T1 JOIN orders AS T2 ON T1.customer\_id  =  T2.customer\_id GROUP BY T1.customer\_id HAVING count(*)  <=  2
\\
\\
% CREATE TABLE Activity (\\
% actid INTEGER PRIMARY KEY,\\
% activity\_name varchar(25)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Activity  LIMIT 3;\\
% actid     activity\_name \\
%   770 Mountain Climbing \\
%   771          Canoeing \\
%   772          Kayaking \\
% */\\
% \\
% CREATE TABLE Participates\_in (\\
% stuid INTEGER,\\
% actid INTEGER,\\
% FOREIGN KEY(stuid) REFERENCES Student(StuID),\\
% FOREIGN KEY(actid) REFERENCES Activity(actid)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Participates\_in  LIMIT 3;\\
% stuid actid \\
%  1001   770 \\
%  1001   771 \\
%  1001   777 \\
% */\\
% \\
% CREATE TABLE Faculty\_Participates\_in (\\
% FacID INTEGER,\\
% actid INTEGER,\\
% FOREIGN KEY(FacID) REFERENCES Faculty(FacID),\\
% FOREIGN KEY(actid) REFERENCES Activity(actid)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Faculty\_Participates\_in  LIMIT 3;\\
% FacID actid \\
%  1082   784 \\
%  1082   785 \\
%  1082   790 \\
% */\\
% \\
% CREATE TABLE Student (\\
% StuID        INTEGER PRIMARY KEY,\\
% LName        VARCHAR(12),\\
% Fname        VARCHAR(12),\\
% Age      INTEGER,\\
% Sex      VARCHAR(1),\\
% Major        INTEGER,\\
% Advisor      INTEGER,\\
% city\_code    VARCHAR(3)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Student  LIMIT 3;\\
% StuID LName  Fname Age Sex Major Advisor city\_code \\
%  1001 Smith  Linda  18   F   600    1121       BAL \\
%  1002   Kim  Tracy  19   F   600    7712       HKG \\
%  1003 Jones Shiela  21   F   600    7792       WAS \\
% */\\
% \\
% CREATE TABLE Faculty (\\
% FacID          INTEGER PRIMARY KEY,\\
% Lname   VARCHAR(15),\\
% Fname   VARCHAR(15),\\
% Rank    VARCHAR(15),\\
% Sex   VARCHAR(1),\\
% Phone   INTEGER,\\
% Room    VARCHAR(5),\\
% Building    VARCHAR(13)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Faculty  LIMIT 3;\\
% FacID    Lname   Fname       Rank Sex Phone Room Building \\
%  1082 Giuliano    Mark Instructor   M  2424  224      NEB \\
%  1121 Goodrich Michael  Professor   M  3593  219      NEB \\
%  1148   Masson  Gerald  Professor   M  3402 224B      NEB \\
% */\\
% \\
% Q: Which rank has the smallest number of faculty members?\\
% A: SELECT rank FROM Faculty GROUP BY rank ORDER BY count(*) ASC LIMIT 1\\
\\
CREATE TABLE stadium (\\
Stadium\_ID int,\\
Location text,\\
Name text,\\
Capacity int,\\
Highest int,\\
Lowest int,\\
Average int,\\
PRIMARY KEY (Stadium\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM stadium  LIMIT 3;\\
Stadium\_ID     Location            Name Capacity Highest Lowest Average \\
         1 Raith Rovers    Stark's Park    10104    4812   1294    2106 \\
         2   Ayr United   Somerset Park    11998    2363   1057    1477 \\
         3    East Fife Bayview Stadium     2000    1980    533     864 \\
*/\\
\\
CREATE TABLE singer (\\
Singer\_ID int,\\
Name text,\\
Country text,\\
Song\_Name text,\\
Song\_release\_year text,\\
Age int,\\
Is\_male bool,\\
PRIMARY KEY (Singer\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM singer  LIMIT 3;\\
Singer\_ID         Name       Country Song\_Name Song\_release\_year Age Is\_male \\
        1    Joe Sharp   Netherlands       You              1992  52       F \\
        2    Timbaland United States Dangerous              2008  32       T \\
        3 Justin Brown        France    Hey Oh              2013  29       T \\
*/\\
\\
CREATE TABLE concert (\\
concert\_ID int,\\
concert\_Name text,\\
Theme text,\\
Stadium\_ID text,\\
Year text,\\
PRIMARY KEY (concert\_ID),\\
FOREIGN KEY (Stadium\_ID) REFERENCES stadium(Stadium\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM concert  LIMIT 3;\\
concert\_ID   concert\_Name         Theme Stadium\_ID Year \\
         1      Auditions   Free choice          1 2014 \\
         2 Super bootcamp Free choice 2          2 2014 \\
         3    Home Visits Bleeding Love          2 2015 \\
*/\\
\\
CREATE TABLE singer\_in\_concert (\\
concert\_ID int,\\
Singer\_ID text,\\
PRIMARY KEY (concert\_ID,Singer\_ID),\\
FOREIGN KEY (concert\_ID) REFERENCES concert(concert\_ID),\\
FOREIGN KEY (Singer\_ID) REFERENCES singer(Singer\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM singer\_in\_concert  LIMIT 3;\\
concert\_ID Singer\_ID \\
         1         2 \\
         1         3 \\
         1         5 \\
*/\\
\\
Q: How many singers do we have?\\
A: \\

==> app_example/ctb_least_to_most_fig.tex <==
% \noindent \textbf{\LTM + Create Table + Select 3 prompting (Problem Reduction)} 

\tiny\texttt{\input{app_example/ctb_least_to_most_p1.tex}
}
% \fontsize{10}{12}

\begin{figure}[ht]
    \caption{An example prompt under least-to-most + Create Table + Select 3 prompting (problem reduction) for 1-shot on Spider}
    \label{fig:api_standard}
\end{figure}



\tiny\texttt{\input{app_example/ctb_least_to_most_p2.tex}}

\begin{figure}[ht]
    % \fontsize{10}{12}
    \caption{An example prompt under least-to-most + Create Table + Select 3 prompting (problem solving) for 1-shot on Spider.}
    \label{fig:api_standard}
\end{figure}


% \noindent \textbf{\LTM + Create Table + Select 3 prompting (Problem Solving)}

% \noindent An example prompt under least-to-most + Create Table + Select 3 prompting (problem solving) for 1-shot on Spider. \\




% \noindent \textbf{\LTM + Create Table + Select 3 prompting (Problem Reduction)} 

% \noindent An example prompt under least-to-most + Create Table + Select 3 prompting (problem reduction) for 1-shot on Spider. \\



% \noindent \textbf{\LTM + Create Table + Select 3 prompting (Problem Solving)}
% \centering

==> app_example/ctb_least_to_most_p1.tex <==
% \noindent \textbf{\LTM + Create Table + Select 3 prompting (Problem Reduction)} 

% \noindent An example prompt under least-to-most + Create Table + Select 3 prompting (problem reduction) for 1-shot on Spider. \\

% An example prompt under standard prompting for 4-shot on Spider
% 


\noindent CREATE TABLE Customers (\\
customer\_id INTEGER PRIMARY KEY,\\
customer\_name VARCHAR(80),\\
customer\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Customers  LIMIT 3;\\
customer\_id customer\_name customer\_details \\
          1      Savannah            rerum \\
          2        George              est \\
          3       Alberto         deleniti \\
*/\\
\\
CREATE TABLE Invoices (\\
invoice\_number INTEGER PRIMARY KEY,\\
invoice\_date DATETIME,\\
invoice\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Invoices  LIMIT 3;\\
invoice\_number        invoice\_date invoice\_details \\
             1 1989-09-03 16:03:05           vitae \\
             2 1989-12-11 16:40:57          magnam \\
             3 1995-10-07 14:13:05              et \\
*/\\
\\
CREATE TABLE Orders (\\
order\_id INTEGER PRIMARY KEY,\\
customer\_id INTEGER NOT NULL,\\
order\_status VARCHAR(10) NOT NULL,\\
date\_order\_placed DATETIME NOT NULL,\\
order\_details VARCHAR(255),\\
FOREIGN KEY (customer\_id ) REFERENCES Customers(customer\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Orders  LIMIT 3;\\
order\_id customer\_id order\_status   date\_order\_placed order\_details \\
       1           2      Shipped 2009-02-21 15:26:19          None \\
       2          11      Shipped 1974-06-24 22:10:26          None \\
       3           4      Shipped 1982-12-29 21:10:11          None \\
*/\\
\\
CREATE TABLE Products (\\
product\_id INTEGER PRIMARY KEY,\\
product\_name VARCHAR(80),\\
product\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Products  LIMIT 3;\\
product\_id product\_name product\_details \\
         1         food            None \\
         2         book            None \\
         3         food            None \\
*/\\
\\
CREATE TABLE Order\_Items (\\
order\_item\_id INTEGER PRIMARY KEY,\\
product\_id INTEGER NOT NULL,\\
order\_id INTEGER NOT NULL,\\
order\_item\_status VARCHAR(10) NOT NULL,\\
order\_item\_details VARCHAR(255),\\
FOREIGN KEY (order\_id ) REFERENCES Orders(order\_id ),\\
FOREIGN KEY (product\_id ) REFERENCES Products(product\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Order\_Items  LIMIT 3;\\
order\_item\_id product\_id order\_id order\_item\_status order\_item\_details \\
            1          4        6            Finish               None \\
            2         15        6            Finish               None \\
            3         12       15            Finish               None \\
*/\\
\\
CREATE TABLE Shipments (\\
shipment\_id INTEGER PRIMARY KEY,\\
order\_id INTEGER NOT NULL,\\
invoice\_number INTEGER NOT NULL,\\
shipment\_tracking\_number VARCHAR(80),\\
shipment\_date DATETIME,\\
other\_shipment\_details VARCHAR(255),\\
FOREIGN KEY (order\_id ) REFERENCES Orders(order\_id ),\\
FOREIGN KEY (invoice\_number ) REFERENCES Invoices(invoice\_number )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Shipments  LIMIT 3;\\
shipment\_id order\_id invoice\_number shipment\_tracking\_number       shipment\_date other\_shipment\_details \\
          1        5             13                     3452 1983-08-13 22:34:11                   None \\
          2        7              2                     0114 1977-11-10 12:11:25                   None \\
          3       10              5                      478 2006-01-17 03:08:05                   None \\
*/\\
\\
CREATE TABLE Shipment\_Items (\\
shipment\_id INTEGER NOT NULL,\\
order\_item\_id INTEGER NOT NULL,\\
FOREIGN KEY (order\_item\_id ) REFERENCES Order\_Items(order\_item\_id ),\\
FOREIGN KEY (shipment\_id ) REFERENCES Shipments(shipment\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Shipment\_Items  LIMIT 3;\\
shipment\_id order\_item\_id \\
         11            12 \\
         10            15 \\
         10            12 \\
*/\\
\\
\\
To answer the question “What are the names of the customers who have made two or less orders?”, we need to know: “What are the names of the customers?”, “What are the names of the customers who have made orders?”. 
\\
% \\
% \\CREATE TABLE grapes (\\
% ID INTEGER PRIMARY KEY,\\
% Grape TEXT UNIQUE,\\
% Color TEXT\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM grapes  LIMIT 3;\\
% ID               Grape Color \\
%  1             Barbera   Red \\
%  2      Cabernet Franc   Red \\
%  3 Cabernet Sauvingnon   Red \\
%  */\\
% \\
% CREATE TABLE appellations (\\
% No INTEGER PRIMARY KEY,\\
% Appelation TEXT UNIQUE,\\
% County TEXT,\\
% State TEXT,\\
% Area TEXT,\\
% isAVA TEXT\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM appellations  LIMIT 3;\\
% No                       Appelation County      State             Area isAVA \\
%  1                 Alexander Valley Sonoma California      North Coast   Yes \\
%  2                    Amador County Amador California Sierra Foothills    No \\
%  3 Amador-Mendocino-Sonoma Counties    N/A California              N/A    No \\
%  */\\
% \\
% CREATE TABLE wine (\\
% No INTEGER,\\
% Grape TEXT,\\
% Winery TEXT,\\
% Appelation TEXT,\\
% State TEXT,\\
% Name TEXT,\\
% Year INTEGER,\\
% Price INTEGER,\\
% Score INTEGER,\\
% Cases INTEGER,\\
% Drink TEXT,\\
% FOREIGN KEY (Grape) REFERENCES grapes(Grape),\\
% FOREIGN KEY (Appelation) REFERENCES appellations(Appelation)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM wine  LIMIT 3;\\
% No     Grape           Winery  Appelation      State               Name Year Price Score Cases Drink \\
%  1 Zinfandel     Robert Biale  St. Helena California Old Kraft Vineyard 2008    44    93   275   now \\
%  2 Zinfandel Chiarello Family Napa Valley California              Giana 2008    35    93   480   now \\
%  3 Zinfandel     Robert Biale Napa Valley California      Black Chicken 2008    40    91  2700  2012 \\
%  */\\
% \\
% \\
% To answer the question “How many wines are produced at Robert Biale winery?”, we need to know: .
% \\
% \\
% \\
% CREATE TABLE Activity (\\
% actid INTEGER PRIMARY KEY,\\
% activity\_name varchar(25)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Activity  LIMIT 3;\\
% actid     activity\_name \\
%   770 Mountain Climbing \\
%   771          Canoeing \\
%   772          Kayaking \\
%   */\\
% \\
% CREATE TABLE Participates\_in (\\
% stuid INTEGER,\\
% actid INTEGER,\\
% FOREIGN KEY(stuid) REFERENCES Student(StuID),\\
% FOREIGN KEY(actid) REFERENCES Activity(actid)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Participates\_in  LIMIT 3;\\
% stuid actid \\
%  1001   770 \\
%  1001   771 \\
%  1001   777 \\
%  */\\
% \\
% CREATE TABLE Faculty\_Participates\_in (\\
% FacID INTEGER,\\
% actid INTEGER,\\
% FOREIGN KEY(FacID) REFERENCES Faculty(FacID),\\
% FOREIGN KEY(actid) REFERENCES Activity(actid)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Faculty\_Participates\_in  LIMIT 3;\\
% FacID actid \\
%  1082   784 \\
%  1082   785 \\
%  1082   790 \\
%  */\\
% \\
% CREATE TABLE Student (\\
% StuID        INTEGER PRIMARY KEY,\\
% LName        VARCHAR(12),\\
% Fname        VARCHAR(12),\\
% Age      INTEGER,\\
% Sex      VARCHAR(1),\\
% Major        INTEGER,\\
% Advisor      INTEGER,\\
% city\_code    VARCHAR(3)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Student  LIMIT 3;\\
% StuID LName  Fname Age Sex Major Advisor city\_code \\
%  1001 Smith  Linda  18   F   600    1121       BAL \\
%  1002   Kim  Tracy  19   F   600    7712       HKG \\
%  1003 Jones Shiela  21   F   600    7792       WAS \\
%  */\\
% \\
% CREATE TABLE Faculty (\\
% FacID          INTEGER PRIMARY KEY,\\
% Lname   VARCHAR(15),\\
% Fname   VARCHAR(15),\\
% Rank    VARCHAR(15),\\
% Sex   VARCHAR(1),\\
% Phone   INTEGER,\\
% Room    VARCHAR(5),\\
% Building    VARCHAR(13)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Faculty  LIMIT 3;\\
% FacID    Lname   Fname       Rank Sex Phone Room Building \\
%  1082 Giuliano    Mark Instructor   M  2424  224      NEB \\
%  1121 Goodrich Michael  Professor   M  3593  219      NEB \\
%  1148   Masson  Gerald  Professor   M  3402 224B      NEB \\
%  */\\
% \\
% \\
% To answer the question “Which rank has the smallest number of faculty members?”, we need to know: .\\
\\
\\
CREATE TABLE stadium (\\
Stadium\_ID int,\\
Location text,\\
Name text,\\
Capacity int,\\
Highest int,\\
Lowest int,\\
Average int,\\
PRIMARY KEY (Stadium\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM stadium  LIMIT 3;\\
Stadium\_ID     Location            Name Capacity Highest Lowest Average \\
         1 Raith Rovers    Stark's Park    10104    4812   1294    2106 \\
         2   Ayr United   Somerset Park    11998    2363   1057    1477 \\
         3    East Fife Bayview Stadium     2000    1980    533     864 \\
         */\\
\\
CREATE TABLE singer (\\
Singer\_ID int,\\
Name text,\\
Country text,\\
Song\_Name text,\\
Song\_release\_year text,\\
Age int,\\
Is\_male bool,\\
PRIMARY KEY (Singer\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM singer  LIMIT 3;\\
Singer\_ID         Name       Country Song\_Name Song\_release\_year Age Is\_male \\
        1    Joe Sharp   Netherlands       You              1992  52       F \\
        2    Timbaland United States Dangerous              2008  32       T \\
        3 Justin Brown        France    Hey Oh              2013  29       T \\
        */\\
\\
CREATE TABLE concert (\\
concert\_ID int,\\
concert\_Name text,\\
Theme text,\\
Stadium\_ID text,\\
Year text,\\
PRIMARY KEY (concert\_ID),\\
FOREIGN KEY (Stadium\_ID) REFERENCES stadium(Stadium\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM concert  LIMIT 3;\\
concert\_ID   concert\_Name         Theme Stadium\_ID Year \\
         1      Auditions   Free choice          1 2014 \\
         2 Super bootcamp Free choice 2          2 2014 \\
         3    Home Visits Bleeding Love          2 2015 \\
         */\\
\\
CREATE TABLE singer\_in\_concert (\\
concert\_ID int,\\
Singer\_ID text,\\
PRIMARY KEY (concert\_ID,Singer\_ID),\\
FOREIGN KEY (concert\_ID) REFERENCES concert(concert\_ID),\\
FOREIGN KEY (Singer\_ID) REFERENCES singer(Singer\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM singer\_in\_concert  LIMIT 3;\\
concert\_ID Singer\_ID \\
         1         2 \\
         1         3 \\
         1         5 \\
         */\\
\\
\\
To answer the question “How many singers do we have?”, we need to know: \\
\\

==> app_example/ctb_least_to_most_p2.tex <==
% \noindent \textbf{\LTM + Create Table + Select 3 prompting (Problem Solving)}

% \noindent An example prompt under least-to-most + Create Table + Select 3 prompting (problem solving) for 1-shot on Spider. \\


% \noindent An example prompt under \LTM + Create Table + Select 3 prompting (decomposition) for 1-shot on Spider. 



\noindent CREATE TABLE Customers (\\
customer\_id INTEGER PRIMARY KEY,\\
customer\_name VARCHAR(80),\\
customer\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Customers  LIMIT 3;\\
customer\_id customer\_name customer\_details \\
          1      Savannah            rerum \\
          2        George              est \\
          3       Alberto         deleniti \\
*/\\
\\
CREATE TABLE Invoices (\\
invoice\_number INTEGER PRIMARY KEY,\\
invoice\_date DATETIME,\\
invoice\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Invoices  LIMIT 3;\\
invoice\_number        invoice\_date invoice\_details \\
             1 1989-09-03 16:03:05           vitae \\
             2 1989-12-11 16:40:57          magnam \\
             3 1995-10-07 14:13:05              et \\
*/\\
\\
CREATE TABLE Orders (\\
order\_id INTEGER PRIMARY KEY,\\
customer\_id INTEGER NOT NULL,\\
order\_status VARCHAR(10) NOT NULL,\\
date\_order\_placed DATETIME NOT NULL,\\
order\_details VARCHAR(255),\\
FOREIGN KEY (customer\_id ) REFERENCES Customers(customer\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Orders  LIMIT 3;\\
order\_id customer\_id order\_status   date\_order\_placed order\_details \\
       1           2      Shipped 2009-02-21 15:26:19          None \\
       2          11      Shipped 1974-06-24 22:10:26          None \\
       3           4      Shipped 1982-12-29 21:10:11          None \\
*/\\
\\
CREATE TABLE Products (\\
product\_id INTEGER PRIMARY KEY,\\
product\_name VARCHAR(80),\\
product\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Products  LIMIT 3;\\
product\_id product\_name product\_details \\
         1         food            None \\
         2         book            None \\
         3         food            None \\
*/\\
\\
CREATE TABLE Order\_Items (\\
order\_item\_id INTEGER PRIMARY KEY,\\
product\_id INTEGER NOT NULL,\\
order\_id INTEGER NOT NULL,\\
order\_item\_status VARCHAR(10) NOT NULL,\\
order\_item\_details VARCHAR(255),\\
FOREIGN KEY (order\_id ) REFERENCES Orders(order\_id ),\\
FOREIGN KEY (product\_id ) REFERENCES Products(product\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Order\_Items  LIMIT 3;\\
order\_item\_id product\_id order\_id order\_item\_status order\_item\_details \\
            1          4        6            Finish               None \\
            2         15        6            Finish               None \\
            3         12       15            Finish               None \\
*/\\
\\
CREATE TABLE Shipments (\\
shipment\_id INTEGER PRIMARY KEY,\\
order\_id INTEGER NOT NULL,\\
invoice\_number INTEGER NOT NULL,\\
shipment\_tracking\_number VARCHAR(80),\\
shipment\_date DATETIME,\\
other\_shipment\_details VARCHAR(255),\\
FOREIGN KEY (order\_id ) REFERENCES Orders(order\_id ),\\
FOREIGN KEY (invoice\_number ) REFERENCES Invoices(invoice\_number )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Shipments  LIMIT 3;\\
shipment\_id order\_id invoice\_number shipment\_tracking\_number       shipment\_date other\_shipment\_details \\
          1        5             13                     3452 1983-08-13 22:34:11                   None \\
          2        7              2                     0114 1977-11-10 12:11:25                   None \\
          3       10              5                      478 2006-01-17 03:08:05                   None \\
*/\\
\\
CREATE TABLE Shipment\_Items (\\
shipment\_id INTEGER NOT NULL,\\
order\_item\_id INTEGER NOT NULL,\\
FOREIGN KEY (order\_item\_id ) REFERENCES Order\_Items(order\_item\_id ),\\
FOREIGN KEY (shipment\_id ) REFERENCES Shipments(shipment\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Shipment\_Items  LIMIT 3;\\
shipment\_id order\_item\_id \\
         11            12 \\
         10            15 \\
         10            12 \\
*/\\
\\
Q: What are the names of the customers?\\
A: SELECT customer\_name FROM customers\\
\\
Q: What are the names of the customers who have made orders?\\
A: SELECT T1.customer\_name FROM customers AS T1 JOIN orders AS T2 ON T1.customer\_id  =  T2.customer\_id\\
\\
Q: What are the names of the customers who have made two or less orders?\\
A: SELECT T1.customer\_name FROM customers AS T1 JOIN orders AS T2 ON T1.customer\_id  =  T2.customer\_id GROUP BY T1.customer\_id HAVING count(*)  <=  2
\\
\\
% CREATE TABLE Activity (\\
% actid INTEGER PRIMARY KEY,\\
% activity\_name varchar(25)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Activity  LIMIT 3;\\
% actid     activity\_name \\
%   770 Mountain Climbing \\
%   771          Canoeing \\
%   772          Kayaking \\
% */\\
% \\
% CREATE TABLE Participates\_in (\\
% stuid INTEGER,\\
% actid INTEGER,\\
% FOREIGN KEY(stuid) REFERENCES Student(StuID),\\
% FOREIGN KEY(actid) REFERENCES Activity(actid)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Participates\_in  LIMIT 3;\\
% stuid actid \\
%  1001   770 \\
%  1001   771 \\
%  1001   777 \\
% */\\
% \\
% CREATE TABLE Faculty\_Participates\_in (\\
% FacID INTEGER,\\
% actid INTEGER,\\
% FOREIGN KEY(FacID) REFERENCES Faculty(FacID),\\
% FOREIGN KEY(actid) REFERENCES Activity(actid)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Faculty\_Participates\_in  LIMIT 3;\\
% FacID actid \\
%  1082   784 \\
%  1082   785 \\
%  1082   790 \\
% */\\
% \\
% CREATE TABLE Student (\\
% StuID        INTEGER PRIMARY KEY,\\
% LName        VARCHAR(12),\\
% Fname        VARCHAR(12),\\
% Age      INTEGER,\\
% Sex      VARCHAR(1),\\
% Major        INTEGER,\\
% Advisor      INTEGER,\\
% city\_code    VARCHAR(3)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Student  LIMIT 3;\\
% StuID LName  Fname Age Sex Major Advisor city\_code \\
%  1001 Smith  Linda  18   F   600    1121       BAL \\
%  1002   Kim  Tracy  19   F   600    7712       HKG \\
%  1003 Jones Shiela  21   F   600    7792       WAS \\
% */\\
% \\
% CREATE TABLE Faculty (\\
% FacID          INTEGER PRIMARY KEY,\\
% Lname   VARCHAR(15),\\
% Fname   VARCHAR(15),\\
% Rank    VARCHAR(15),\\
% Sex   VARCHAR(1),\\
% Phone   INTEGER,\\
% Room    VARCHAR(5),\\
% Building    VARCHAR(13)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM Faculty  LIMIT 3;\\
% FacID    Lname   Fname       Rank Sex Phone Room Building \\
%  1082 Giuliano    Mark Instructor   M  2424  224      NEB \\
%  1121 Goodrich Michael  Professor   M  3593  219      NEB \\
%  1148   Masson  Gerald  Professor   M  3402 224B      NEB \\
% */\\
% \\
% Q: Which rank has the smallest number of faculty members?\\
% A: SELECT rank FROM Faculty GROUP BY rank ORDER BY count(*) ASC LIMIT 1\\
\\
CREATE TABLE stadium (\\
Stadium\_ID int,\\
Location text,\\
Name text,\\
Capacity int,\\
Highest int,\\
Lowest int,\\
Average int,\\
PRIMARY KEY (Stadium\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM stadium  LIMIT 3;\\
Stadium\_ID     Location            Name Capacity Highest Lowest Average \\
         1 Raith Rovers    Stark's Park    10104    4812   1294    2106 \\
         2   Ayr United   Somerset Park    11998    2363   1057    1477 \\
         3    East Fife Bayview Stadium     2000    1980    533     864 \\
*/\\
\\
CREATE TABLE singer (\\
Singer\_ID int,\\
Name text,\\
Country text,\\
Song\_Name text,\\
Song\_release\_year text,\\
Age int,\\
Is\_male bool,\\
PRIMARY KEY (Singer\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM singer  LIMIT 3;\\
Singer\_ID         Name       Country Song\_Name Song\_release\_year Age Is\_male \\
        1    Joe Sharp   Netherlands       You              1992  52       F \\
        2    Timbaland United States Dangerous              2008  32       T \\
        3 Justin Brown        France    Hey Oh              2013  29       T \\
*/\\
\\
CREATE TABLE concert (\\
concert\_ID int,\\
concert\_Name text,\\
Theme text,\\
Stadium\_ID text,\\
Year text,\\
PRIMARY KEY (concert\_ID),\\
FOREIGN KEY (Stadium\_ID) REFERENCES stadium(Stadium\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM concert  LIMIT 3;\\
concert\_ID   concert\_Name         Theme Stadium\_ID Year \\
         1      Auditions   Free choice          1 2014 \\
         2 Super bootcamp Free choice 2          2 2014 \\
         3    Home Visits Bleeding Love          2 2015 \\
*/\\
\\
CREATE TABLE singer\_in\_concert (\\
concert\_ID int,\\
Singer\_ID text,\\
PRIMARY KEY (concert\_ID,Singer\_ID),\\
FOREIGN KEY (concert\_ID) REFERENCES concert(concert\_ID),\\
FOREIGN KEY (Singer\_ID) REFERENCES singer(Singer\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM singer\_in\_concert  LIMIT 3;\\
concert\_ID Singer\_ID \\
         1         2 \\
         1         3 \\
         1         5 \\
*/\\
\\
Q: How many singers do we have?\\
A: \\

==> app_example/ctb_qdemp.tex <==
% \noindent \textbf{\QDEMP + Create Table + Select 3 Prompting} 

% \noindent An example prompt under \QDEMP + Create Table + Select 3 prompting for 1-shot on Spider. \\

% An example prompt under standard prompting for 4-shot on Spider.

\noindent CREATE TABLE Customers (\\
customer\_id INTEGER PRIMARY KEY,\\
customer\_name VARCHAR(80),\\
customer\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Customers  LIMIT 3;\\
customer\_id customer\_name customer\_details \\
          1      Savannah            rerum \\
          2        George              est \\
          3       Alberto         deleniti \\
*/\\
\\
CREATE TABLE Invoices (\\
invoice\_number INTEGER PRIMARY KEY,\\
invoice\_date DATETIME,\\
invoice\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Invoices  LIMIT 3;\\
invoice\_number        invoice\_date invoice\_details \\
             1 1989-09-03 16:03:05           vitae \\
             2 1989-12-11 16:40:57          magnam \\
             3 1995-10-07 14:13:05              et \\
*/\\
\\
CREATE TABLE Orders (\\
order\_id INTEGER PRIMARY KEY,\\
customer\_id INTEGER NOT NULL,\\
order\_status VARCHAR(10) NOT NULL,\\
date\_order\_placed DATETIME NOT NULL,\\
order\_details VARCHAR(255),\\
FOREIGN KEY (customer\_id ) REFERENCES Customers(customer\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Orders  LIMIT 3;\\
order\_id customer\_id order\_status   date\_order\_placed order\_details \\
       1           2      Shipped 2009-02-21 15:26:19          None \\
       2          11      Shipped 1974-06-24 22:10:26          None \\
       3           4      Shipped 1982-12-29 21:10:11          None \\
*/\\
\\
CREATE TABLE Products (\\
product\_id INTEGER PRIMARY KEY,\\
product\_name VARCHAR(80),\\
product\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Products  LIMIT 3;\\
product\_id product\_name product\_details \\
         1         food            None \\
         2         book            None \\
         3         food            None \\
*/\\
\\
CREATE TABLE Order\_Items (\\
order\_item\_id INTEGER PRIMARY KEY,\\
product\_id INTEGER NOT NULL,\\
order\_id INTEGER NOT NULL,\\
order\_item\_status VARCHAR(10) NOT NULL,\\
order\_item\_details VARCHAR(255),\\
FOREIGN KEY (order\_id ) REFERENCES Orders(order\_id ),\\
FOREIGN KEY (product\_id ) REFERENCES Products(product\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Order\_Items  LIMIT 3;\\
order\_item\_id product\_id order\_id order\_item\_status order\_item\_details \\
            1          4        6            Finish               None \\
            2         15        6            Finish               None \\
            3         12       15            Finish               None \\
*/\\
\\
CREATE TABLE Shipments (\\
shipment\_id INTEGER PRIMARY KEY,\\
order\_id INTEGER NOT NULL,\\
invoice\_number INTEGER NOT NULL,\\
shipment\_tracking\_number VARCHAR(80),\\
shipment\_date DATETIME,\\
other\_shipment\_details VARCHAR(255),\\
FOREIGN KEY (order\_id ) REFERENCES Orders(order\_id ),\\
FOREIGN KEY (invoice\_number ) REFERENCES Invoices(invoice\_number )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Shipments  LIMIT 3;\\
shipment\_id order\_id invoice\_number shipment\_tracking\_number       shipment\_date other\_shipment\_details \\
          1        5             13                     3452 1983-08-13 22:34:11                   None \\
          2        7              2                     0114 1977-11-10 12:11:25                   None \\
          3       10              5                      478 2006-01-17 03:08:05                   None \\
*/\\
\\
CREATE TABLE Shipment\_Items (\\
shipment\_id INTEGER NOT NULL,\\
order\_item\_id INTEGER NOT NULL,\\
FOREIGN KEY (order\_item\_id ) REFERENCES Order\_Items(order\_item\_id ),\\
FOREIGN KEY (shipment\_id ) REFERENCES Shipments(shipment\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Shipment\_Items  LIMIT 3;\\
shipment\_id order\_item\_id \\
         11            12 \\
         10            15 \\
         10            12 \\
*/\\
\\
\#\#\# Question: What are the names of the customers who have made two or less orders?\\
decompose the question\\
\\
1. What are the names of the customers?\\
2. What are the names of the customers who have made orders?\\
3. What are the names of the customers who have made two or less orders?\\
\\
\# Thus, the answer for the question is: What are the names of the customers who have made two or less orders?\\
SELECT T2.customer\_name FROM orders AS T1 JOIN customers AS T2 ON T1.customer\_id = T2.customer\_id GROUP BY T2.customer\_id HAVING count(*)  <=  2\\
\\
% \noindent CREATE TABLE grapes (\\
% ID INTEGER PRIMARY KEY,\\
% Grape TEXT UNIQUE,\\
% Color TEXT\\
% )\\ 
% /*\\
% 3 example rows:\\
% SELECT * FROM grapes  LIMIT 3;\\
% ID               Grape Color \\
%  1             Barbera   Red \\
%  2      Cabernet Franc   Red \\
%  3 Cabernet Sauvingnon   Red \\
% */\\
% \\
% CREATE TABLE appellations (\\
% No INTEGER PRIMARY KEY,\\
% Appelation TEXT UNIQUE,\\
% County TEXT,\\
% State TEXT,\\
% Area TEXT,\\
% isAVA TEXT\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM appellations  LIMIT 3;\\
% No                       Appelation County      State             Area isAVA \\
%  1                 Alexander Valley Sonoma California      North Coast   Yes \\
%  2                    Amador County Amador California Sierra Foothills    No \\
%  3 Amador-Mendocino-Sonoma Counties    N/A California              N/A    No \\
% */\\
% \\
% CREATE TABLE wine (\\
% No INTEGER,\\
% Grape TEXT,\\
% Winery TEXT,\\
% Appelation TEXT,\\
% State TEXT,\\
% Name TEXT,\\
% Year INTEGER,\\
% Price INTEGER,\\
% Score INTEGER,\\
% Cases INTEGER,\\
% Drink TEXT,\\
% FOREIGN KEY (Grape) REFERENCES grapes(Grape),\\
% FOREIGN KEY (Appelation) REFERENCES appellations(Appelation)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM wine  LIMIT 3;\\
% No     Grape           Winery  Appelation      State               Name Year Price Score Cases Drink \\
%  1 Zinfandel     Robert Biale  St. Helena California Old Kraft Vineyard 2008    44    93   275   now \\
%  2 Zinfandel Chiarello Family Napa Valley California              Giana 2008    35    93   480   now \\
%  3 Zinfandel     Robert Biale Napa Valley California      Black Chicken 2008    40    91  2700  2012 \\
% */\\
% \\
% \#\#\# Question: How many wines are produced at Robert Biale winery?\\
% decompose the question\\
% \\
% 1. How many wines are produced at Robert Biale winery?\\
% \\
% \# Thus, the answer for the question is: How many wines are produced at Robert Biale winery?\\
% SELECT count(*) FROM WINE WHERE Winery  =  "Robert Biale"\\
\\
% % CREATE TABLE Activity (\\
% % actid INTEGER PRIMARY KEY,\\
% % activity\_name varchar(25)\\
% % )\\
% % /*\\
% % 3 example rows:\\
% % SELECT * FROM Activity  LIMIT 3;\\
% % actid     activity\_name \\
% %   770 Mountain Climbing \\
% %   771          Canoeing \\
% %   772          Kayaking \\
% % */\\
% % \\
% % CREATE TABLE Participates\_in (\\
% % stuid INTEGER,\\
% % actid INTEGER,\\
% % FOREIGN KEY(stuid) REFERENCES Student(StuID),\\
% % FOREIGN KEY(actid) REFERENCES Activity(actid)\\
% % )\\
% % /*\\
% % 3 example rows:\\
% % SELECT * FROM Participates\_in  LIMIT 3;\\
% % stuid actid \\
% %  1001   770 \\
% %  1001   771 \\
% %  1001   777 \\
% % */\\
% % \\
% % CREATE TABLE Faculty\_Participates\_in (\\
% % FacID INTEGER,\\
% % actid INTEGER,\\
% % FOREIGN KEY(FacID) REFERENCES Faculty(FacID),\\
% % FOREIGN KEY(actid) REFERENCES Activity(actid)\\
% % )\\
% % /*\\
% % 3 example rows:\\
% % SELECT * FROM Faculty\_Participates\_in  LIMIT 3;\\
% % FacID actid \\
% %  1082   784 \\
% %  1082   785 \\
% %  1082   790 \\
% % */\\
% % \\
% % CREATE TABLE Student (\\
% % StuID        INTEGER PRIMARY KEY,\\
% % LName        VARCHAR(12),\\
% % Fname        VARCHAR(12),\\
% % Age      INTEGER,\\
% % Sex      VARCHAR(1),\\
% % Major        INTEGER,\\
% % Advisor      INTEGER,\\
% % city\_code    VARCHAR(3)\\
% % )\\
% % /*\\
% % 3 example rows:\\
% % SELECT * FROM Student  LIMIT 3;\\
% % StuID LName  Fname Age Sex Major Advisor city\_code \\
% %  1001 Smith  Linda  18   F   600    1121       BAL \\
% %  1002   Kim  Tracy  19   F   600    7712       HKG \\
% %  1003 Jones Shiela  21   F   600    7792       WAS \\
% % */\\
% % \\
% % CREATE TABLE Faculty (\\
% % FacID          INTEGER PRIMARY KEY,\\
% % Lname   VARCHAR(15),\\
% % Fname   VARCHAR(15),\\
% % Rank    VARCHAR(15),\\
% % Sex   VARCHAR(1),\\
% % Phone   INTEGER,\\
% % Room    VARCHAR(5),\\
% % Building    VARCHAR(13)\\
% % )\\
% % /*\\
% % 3 example rows:\\
% % SELECT * FROM Faculty  LIMIT 3;\\
% % FacID    Lname   Fname       Rank Sex Phone Room Building \\
% %  1082 Giuliano    Mark Instructor   M  2424  224      NEB \\
% %  1121 Goodrich Michael  Professor   M  3593  219      NEB \\
% %  1148   Masson  Gerald  Professor   M  3402 224B      NEB \\
% % */\\
% % \\
% % \#\#\# Question: Which rank has the smallest number of faculty members?\\
% % decompose the question\\
% % \\
% % 1. Which rank has the smallest number of faculty members?\\
% % \\
% % \# Thus, the answer for the question is: Which rank has the smallest number of faculty members?\\
% % SELECT rank FROM Faculty GROUP BY rank ORDER BY count(*) ASC LIMIT 1\\
% \\
CREATE TABLE stadium (\\
Stadium\_ID int,\\
Location text,\\
Name text,\\
Capacity int,\\
Highest int,\\
Lowest int,\\
Average int,\\
PRIMARY KEY (Stadium\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM stadium  LIMIT 3;\\
Stadium\_ID     Location            Name Capacity Highest Lowest Average \\
         1 Raith Rovers    Stark's Park    10104    4812   1294    2106 \\
         2   Ayr United   Somerset Park    11998    2363   1057    1477 \\
         3    East Fife Bayview Stadium     2000    1980    533     864 \\
*/\\
\\
CREATE TABLE singer (\\
Singer\_ID int,\\
Name text,\\
Country text,\\
Song\_Name text,\\
Song\_release\_year text,\\
Age int,\\
Is\_male bool,\\
PRIMARY KEY (Singer\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM singer  LIMIT 3;\\
Singer\_ID         Name       Country Song\_Name Song\_release\_year Age Is\_male \\
        1    Joe Sharp   Netherlands       You              1992  52       F \\
        2    Timbaland United States Dangerous              2008  32       T \\
        3 Justin Brown        France    Hey Oh              2013  29       T \\
*/\\
\\
CREATE TABLE concert (\\
concert\_ID int,\\
concert\_Name text,\\
Theme text,\\
Stadium\_ID text,\\
Year text,\\
PRIMARY KEY (concert\_ID),\\
FOREIGN KEY (Stadium\_ID) REFERENCES stadium(Stadium\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM concert  LIMIT 3;\\
concert\_ID   concert\_Name         Theme Stadium\_ID Year \\
         1      Auditions   Free choice          1 2014 \\
         2 Super bootcamp Free choice 2          2 2014 \\
         3    Home Visits Bleeding Love          2 2015 \\
*/\\
\\
CREATE TABLE singer\_in\_concert (\\
concert\_ID int,\\
Singer\_ID text,\\
PRIMARY KEY (concert\_ID,Singer\_ID),\\
FOREIGN KEY (concert\_ID) REFERENCES concert(concert\_ID),\\
FOREIGN KEY (Singer\_ID) REFERENCES singer(Singer\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM singer\_in\_concert  LIMIT 3;\\
concert\_ID Singer\_ID \\
         1         2 \\
         1         3 \\
         1         5 \\
*/\\
\\
\#\#\# Question: How many singers do we have?\\
decompose the question \\

==> app_example/ctb_qdemp_fig.tex <==
% \noindent \textbf{\QDEMP + Create Table + Select 3 Prompting} 
% \centering
\tiny\texttt{\input{app_example/ctb_qdemp.tex}
}

\begin{figure}[ht]
    \caption{An example prompt under \QDEMP + Create Table + Select 3 prompting for 1-shot on Spider.}
    \label{fig:api_standard}
\end{figure}



% \noindent \textbf{\QDEMP + Create Table + Select 3 Prompting} 

% \noindent An example prompt under \QDEMP + Create Table + Select 3 prompting for 1-shot on Spider. \\

==> app_example/ctb_qdemp_intercol.tex <==
% \noindent \textbf{\QDEMPTB + Create Table + Select 3 Prompting} 

% \noindent An example prompt under \QDEMPTB + Create Table + Select 3 Prompting for 1-shot on Spider. \\

% An example prompt under \QDEMP + Create Table + Select 3 prompting for 1-shot on Spider.

\noindent CREATE TABLE Customers (\\
customer\_id INTEGER PRIMARY KEY,\\
customer\_name VARCHAR(80),\\
customer\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Customers  LIMIT 3;\\
customer\_id customer\_name customer\_details \\
          1      Savannah            rerum \\
          2        George              est \\
          3       Alberto         deleniti \\
*/\\
\\
CREATE TABLE Invoices (\\
invoice\_number INTEGER PRIMARY KEY,\\
invoice\_date DATETIME,\\
invoice\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Invoices  LIMIT 3;\\
invoice\_number        invoice\_date invoice\_details \\
             1 1989-09-03 16:03:05           vitae \\
             2 1989-12-11 16:40:57          magnam \\
             3 1995-10-07 14:13:05              et \\
*/\\
\\
CREATE TABLE Orders (\\
order\_id INTEGER PRIMARY KEY,\\
customer\_id INTEGER NOT NULL,\\
order\_status VARCHAR(10) NOT NULL,\\
date\_order\_placed DATETIME NOT NULL,\\
order\_details VARCHAR(255),\\
FOREIGN KEY (customer\_id ) REFERENCES Customers(customer\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Orders  LIMIT 3;\\
order\_id customer\_id order\_status   date\_order\_placed order\_details \\
       1           2      Shipped 2009-02-21 15:26:19          None \\
       2          11      Shipped 1974-06-24 22:10:26          None \\
       3           4      Shipped 1982-12-29 21:10:11          None \\
*/\\
\\
CREATE TABLE Products (\\
product\_id INTEGER PRIMARY KEY,\\
product\_name VARCHAR(80),\\
product\_details VARCHAR(255)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Products  LIMIT 3;\\
product\_id product\_name product\_details \\
         1         food            None \\
         2         book            None \\
         3         food            None \\
*/\\
\\
CREATE TABLE Order\_Items (\\
order\_item\_id INTEGER PRIMARY KEY,\\
product\_id INTEGER NOT NULL,\\
order\_id INTEGER NOT NULL,\\
order\_item\_status VARCHAR(10) NOT NULL,\\
order\_item\_details VARCHAR(255),\\
FOREIGN KEY (order\_id ) REFERENCES Orders(order\_id ),\\
FOREIGN KEY (product\_id ) REFERENCES Products(product\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Order\_Items  LIMIT 3;\\
order\_item\_id product\_id order\_id order\_item\_status order\_item\_details \\
            1          4        6            Finish               None \\
            2         15        6            Finish               None \\
            3         12       15            Finish               None \\
*/\\
\\
CREATE TABLE Shipments (\\
shipment\_id INTEGER PRIMARY KEY,\\
order\_id INTEGER NOT NULL,\\
invoice\_number INTEGER NOT NULL,\\
shipment\_tracking\_number VARCHAR(80),\\
shipment\_date DATETIME,\\
other\_shipment\_details VARCHAR(255),\\
FOREIGN KEY (order\_id ) REFERENCES Orders(order\_id ),\\
FOREIGN KEY (invoice\_number ) REFERENCES Invoices(invoice\_number )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Shipments  LIMIT 3;\\
shipment\_id order\_id invoice\_number shipment\_tracking\_number       shipment\_date other\_shipment\_details \\
          1        5             13                     3452 1983-08-13 22:34:11                   None \\
          2        7              2                     0114 1977-11-10 12:11:25                   None \\
          3       10              5                      478 2006-01-17 03:08:05                   None \\
*/\\
\\
CREATE TABLE Shipment\_Items (\\
shipment\_id INTEGER NOT NULL,\\
order\_item\_id INTEGER NOT NULL,\\
FOREIGN KEY (order\_item\_id ) REFERENCES Order\_Items(order\_item\_id ),\\
FOREIGN KEY (shipment\_id ) REFERENCES Shipments(shipment\_id )\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Shipment\_Items  LIMIT 3;\\
shipment\_id order\_item\_id \\
         11            12 \\
         10            15 \\
         10            12 \\
*/\\
\\
\#\#\# Question: What are the names of the customers who have made two or less orders?\\
decompose the question\\
\\
1. What are the names of the customers?\\
SQL table (column): customers (customer\_name)\\
2. What are the names of the customers who have made orders?\\
SQL table (column): orders (customer\_id)\\
3. What are the names of the customers who have made two or less orders?\\
SQL table (column): customers (customer\_id)\\
\\
\# Thus, the answer for the question is: What are the names of the customers who have made two or less orders?\\
SELECT T2.customer\_name FROM orders AS T1 JOIN customers AS T2 ON T1.customer\_id = T2.customer\_id GROUP BY T2.customer\_id HAVING count(*)  <=  2\\
\\
% CREATE TABLE grapes (\\
% ID INTEGER PRIMARY KEY,\\
% Grape TEXT UNIQUE,\\
% Color TEXT\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM grapes  LIMIT 3;\\
% ID               Grape Color \\
%  1             Barbera   Red \\
%  2      Cabernet Franc   Red \\
%  3 Cabernet Sauvingnon   Red \\
% */\\
% \\
% CREATE TABLE appellations (\\
% No INTEGER PRIMARY KEY,\\
% Appelation TEXT UNIQUE,\\
% County TEXT,\\
% State TEXT,\\
% Area TEXT,\\
% isAVA TEXT\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM appellations  LIMIT 3;\\
% No                       Appelation County      State             Area isAVA \\
%  1                 Alexander Valley Sonoma California      North Coast   Yes \\
%  2                    Amador County Amador California Sierra Foothills    No \\
%  3 Amador-Mendocino-Sonoma Counties    N/A California              N/A    No \\
% */\\
% \\
% CREATE TABLE wine (\\
% No INTEGER,\\
% Grape TEXT,\\
% Winery TEXT,\\
% Appelation TEXT,\\
% State TEXT,\\
% Name TEXT,\\
% Year INTEGER,\\
% Price INTEGER,\\
% Score INTEGER,\\
% Cases INTEGER,\\
% Drink TEXT,\\
% FOREIGN KEY (Grape) REFERENCES grapes(Grape),\\
% FOREIGN KEY (Appelation) REFERENCES appellations(Appelation)\\
% )\\
% /*\\
% 3 example rows:\\
% SELECT * FROM wine  LIMIT 3;\\
% No     Grape           Winery  Appelation      State               Name Year Price Score Cases Drink \\
%  1 Zinfandel     Robert Biale  St. Helena California Old Kraft Vineyard 2008    44    93   275   now \\
%  2 Zinfandel Chiarello Family Napa Valley California              Giana 2008    35    93   480   now \\
%  3 Zinfandel     Robert Biale Napa Valley California      Black Chicken 2008    40    91  2700  2012 \\
% */\\
% \\
% ### Question: How many wines are produced at Robert Biale winery?\\
% decompose the question\\
% \\
% 1. How many wines are produced at Robert Biale winery?\\
% SQL table (column): wine (no)\\
% \\
% # Thus, the answer for the question is: How many wines are produced at Robert Biale winery?\\
% SELECT count(*) FROM WINE WHERE Winery  =  "Robert Biale"\\
% \\
CREATE TABLE Ref\_Template\_Types (\\
Template\_Type\_Code CHAR(15) NOT NULL,\\
Template\_Type\_Description VARCHAR(255) NOT NULL,\\
PRIMARY KEY (Template\_Type\_Code)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Ref\_Template\_Types  LIMIT 3;\\
Template\_Type\_Code Template\_Type\_Description \\
               PPT              Presentation \\
                CV                        CV \\
                AD             Advertisement \\
*/\\
\\
CREATE TABLE Templates (\\
Template\_ID INTEGER NOT NULL,\\
Version\_Number INTEGER NOT NULL,\\
Template\_Type\_Code CHAR(15) NOT NULL,\\
Date\_Effective\_From DATETIME,\\
Date\_Effective\_To DATETIME,\\
Template\_Details VARCHAR(255) NOT NULL,\\
PRIMARY KEY (Template\_ID),\\
FOREIGN KEY (Template\_Type\_Code) REFERENCES Ref\_Template\_Types (Template\_Type\_Code)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Templates  LIMIT 3;\\
Template\_ID Version\_Number Template\_Type\_Code Date\_Effective\_From   Date\_Effective\_To Template\_Details \\
          0              5                 PP 2005-11-12 07:09:48 2008-01-05 14:19:28                  \\
          1              9                 PP 2010-09-24 01:15:11 1999-07-08 03:31:04                  \\
          4              4                 BK 2002-03-02 14:39:49 2001-04-18 09:29:52                  \\
*/\\
\\
CREATE TABLE Documents (\\
Document\_ID INTEGER NOT NULL,\\
Template\_ID INTEGER,\\
Document\_Name VARCHAR(255),\\
Document\_Description VARCHAR(255),\\
Other\_Details VARCHAR(255),\\
PRIMARY KEY (Document\_ID),\\
FOREIGN KEY (Template\_ID) REFERENCES Templates (Template\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Documents  LIMIT 3;\\
Document\_ID Template\_ID      Document\_Name Document\_Description Other\_Details \\
          0           7 Introduction of OS                    n          None \\
          1          25   Understanding DB                    y          None \\
          3           6        Summer Show                    u          None \\
*/\\
\\
CREATE TABLE Paragraphs (\\
Paragraph\_ID INTEGER NOT NULL,\\
Document\_ID INTEGER NOT NULL,\\
Paragraph\_Text VARCHAR(255),\\
Other\_Details VARCHAR(255),\\
PRIMARY KEY (Paragraph\_ID),\\
FOREIGN KEY (Document\_ID) REFERENCES Documents (Document\_ID)\\
)\\
/*\\
3 example rows:\\
SELECT * FROM Paragraphs  LIMIT 3;\\
Paragraph\_ID Document\_ID        Paragraph\_Text Other\_Details \\
           7        2394                 Korea          None \\
           9           3               Somalia          None \\
          65       50123 Palestinian Territory          None \\
*/\\
\\
\#\#\# Question: Return the type code of the template type with the description "Book".\\
decompose the question \\

==> app_example/ctb_qdemp_intercol_fig.tex <==
% \noindent \textbf{\QDEMPTB + Create Table + Select 3 Prompting} 
% \centering
\tiny\texttt{\input{app_example/ctb_qdemp_intercol.tex}
}

\begin{figure}[ht]
    % \fontsize{10}{12}
    \caption{An example prompt under \QDEMPTB + Create Table + Select 3 Prompting for 1-shot on Spider.}
    \label{fig:api_standard}
\end{figure}


% \noindent \textbf{\QDEMPTB + Create Table + Select 3 Prompting} 

% \noindent An example prompt under \QDEMPTB + Create Table + Select 3 Prompting for 1-shot on Spider. \\

==> app_example/ctb_standard.tex <==
% \noindent \textbf{Standard Create Table + Select 3 Prompting} 

% \noindent An example prompt under the standard Create Table + Select 3 prompting for 2-shot on Spider. \\

% An example prompt under standard prompting for 4-shot on Spider


\noindent CREATE TABLE grapes (
\\ID INTEGER PRIMARY KEY,
\\Grape TEXT UNIQUE,
\\Color TEXT
\\)
\\/*
\\3 example rows:
\\SELECT * FROM grapes  LIMIT 3;
\\ID               Grape Color 
\\ 1             Barbera   Red 
\\ 2      Cabernet Franc   Red 
\\ 3 Cabernet Sauvingnon   Red 
\\*/
\\
\\CREATE TABLE appellations (
\\No INTEGER PRIMARY KEY,
\\Appelation TEXT UNIQUE,
\\County TEXT,
\\State TEXT,
\\Area TEXT,
\\isAVA TEXT
\\)
\\/*
\\3 example rows:
\\SELECT * FROM appellations  LIMIT 3;
\\No                       Appelation County      State             Area isAVA 
\\ 1                 Alexander Valley Sonoma California      North Coast   Yes 
\\ 2                    Amador County Amador California Sierra Foothills    No 
\\ 3 Amador-Mendocino-Sonoma Counties    N/A California              N/A    No 
\\*/
\\
\\CREATE TABLE wine (
\\No INTEGER,
\\Grape TEXT,
\\Winery TEXT,
\\Appelation TEXT,
\\State TEXT,
\\Name TEXT,
\\Year INTEGER,
\\Price INTEGER,
\\Score INTEGER,
\\Cases INTEGER,
\\Drink TEXT,
\\FOREIGN KEY (Grape) REFERENCES grapes(Grape),
\\FOREIGN KEY (Appelation) REFERENCES appellations(Appelation)
\\)
\\/*
\\3 example rows:
\\SELECT * FROM wine  LIMIT 3;
\\No     Grape           Winery  Appelation      State               Name Year Price Score Cases Drink 
\\ 1 Zinfandel     Robert Biale  St. Helena California Old Kraft Vineyard 2008    44    93   275   now 
\\ 2 Zinfandel Chiarello Family Napa Valley California              Giana 2008    35    93   480   now 
\\ 3 Zinfandel     Robert Biale Napa Valley California      Black Chicken 2008    40    91  2700  2012 
\\*/
\\
\\-- Using valid SQLite, answer the following questions for the tables provided above.
\\
\\-- How many wines are produced at Robert Biale winery?
\\SELECT count(*) FROM WINE WHERE Winery  =  "Robert Biale"
\\
\\CREATE TABLE Activity (
\\actid INTEGER PRIMARY KEY,
\\activity\_name varchar(25)
\\)
\\/*
\\3 example rows:
\\SELECT * FROM Activity  LIMIT 3;
\\actid     activity\_name 
\\  770 Mountain Climbing 
\\  771          Canoeing 
\\  772          Kayaking 
\\*/
\\
\\CREATE TABLE Participates\_in (
\\stuid INTEGER,
\\actid INTEGER,
\\FOREIGN KEY(stuid) REFERENCES Student(StuID),
\\FOREIGN KEY(actid) REFERENCES Activity(actid)
\\)
\\/*
\\3 example rows:
\\SELECT * FROM Participates\_in  LIMIT 3;
\\stuid actid 
\\ 1001   770 
\\ 1001   771 
\\ 1001   777 
\\*/
\\
\\CREATE TABLE Faculty\_Participates\_in (
\\FacID INTEGER,
\\actid INTEGER,
\\FOREIGN KEY(FacID) REFERENCES Faculty(FacID),
\\FOREIGN KEY(actid) REFERENCES Activity(actid)
\\)
\\/*
\\3 example rows:
\\SELECT * FROM Faculty\_Participates\_in  LIMIT 3;
\\FacID actid 
\\ 1082   784 
\\ 1082   785 
\\ 1082   790 
\\*/
\\
\\CREATE TABLE Student (
\\StuID        INTEGER PRIMARY KEY,
\\LName        VARCHAR(12),
\\Fname        VARCHAR(12),
\\Age      INTEGER,
\\Sex      VARCHAR(1),
\\Major        INTEGER,
\\Advisor      INTEGER,
\\city\_code    VARCHAR(3)
\\)
\\/*
\\3 example rows:
\\SELECT * FROM Student  LIMIT 3;
\\StuID LName  Fname Age Sex Major Advisor city\_code 
\\ 1001 Smith  Linda  18   F   600    1121       BAL 
\\ 1002   Kim  Tracy  19   F   600    7712       HKG 
\\ 1003 Jones Shiela  21   F   600    7792       WAS 
\\*/
\\
\\CREATE TABLE Faculty (
\\FacID 	       INTEGER PRIMARY KEY,
\\Lname		VARCHAR(15),
\\Fname		VARCHAR(15),
\\Rank		VARCHAR(15),
\\Sex		VARCHAR(1),
\\Phone		INTEGER,
\\Room		VARCHAR(5),
\\Building		VARCHAR(13)
\\)
\\/*
\\3 example rows:
\\SELECT * FROM Faculty  LIMIT 3;
\\FacID    Lname   Fname       Rank Sex Phone Room Building 
\\ 1082 Giuliano    Mark Instructor   M  2424  224      NEB 
\\ 1121 Goodrich Michael  Professor   M  3593  219      NEB 
\\ 1148   Masson  Gerald  Professor   M  3402 224B      NEB 
\\*/
\\
\\-- Using valid SQLite, answer the following questions for the tables provided above.
\\
\\-- Which rank has the smallest number of faculty members?
\\SELECT rank FROM Faculty GROUP BY rank ORDER BY count(*) ASC LIMIT 1
\\
\\CREATE TABLE stadium (
\\Stadium\_ID int,
\\Location text,
\\Name text,
\\Capacity int,
\\Highest int,
\\Lowest int,
\\Average int,
\\PRIMARY KEY (Stadium\_ID)
\\)
\\/*
\\3 example rows:
\\SELECT * FROM stadium  LIMIT 3;
\\Stadium\_ID     Location            Name Capacity Highest Lowest Average 
\\         1 Raith Rovers    Stark's Park    10104    4812   1294    2106 
\\         2   Ayr United   Somerset Park    11998    2363   1057    1477 
\\         3    East Fife Bayview Stadium     2000    1980    533     864 
\\*/
\\
\\CREATE TABLE singer (
\\Singer\_ID int,
\\Name text,
\\Country text,
\\Song\_Name text,
\\Song\_release\_year text,
\\Age int,
\\Is\_male bool,
\\PRIMARY KEY (Singer\_ID)
\\)
\\/*
\\3 example rows:
\\SELECT * FROM singer  LIMIT 3;
\\Singer\_ID         Name       Country Song\_Name Song\_release\_year Age Is\_male 
\\        1    Joe Sharp   Netherlands       You              1992  52       F 
\\        2    Timbaland United States Dangerous              2008  32       T 
\\        3 Justin Brown        France    Hey Oh              2013  29       T 
\\*/
\\
\\CREATE TABLE concert (
\\concert\_ID int,
\\concert\_Name text,
\\Theme text,
\\Stadium\_ID text,
\\Year text,
\\PRIMARY KEY (concert\_ID),
\\FOREIGN KEY (Stadium\_ID) REFERENCES stadium(Stadium\_ID)
\\)
\\/*
\\3 example rows:
\\SELECT * FROM concert  LIMIT 3;
\\concert\_ID   concert\_Name         Theme Stadium\_ID Year 
\\         1      Auditions   Free choice          1 2014 
\\         2 Super bootcamp Free choice 2          2 2014 
\\         3    Home Visits Bleeding Love          2 2015 
\\*/
\\
\\CREATE TABLE singer\_in\_concert (
\\concert\_ID int,
\\Singer\_ID text,
\\PRIMARY KEY (concert\_ID,Singer\_ID),
\\FOREIGN KEY (concert\_ID) REFERENCES concert(concert\_ID),
\\FOREIGN KEY (Singer\_ID) REFERENCES singer(Singer\_ID)
\\)
\\/*
\\3 example rows:
\\SELECT * FROM singer\_in\_concert  LIMIT 3;
\\concert\_ID Singer\_ID 
\\         1         2 
\\         1         3 
\\         1         5 
\\*/
\\
\\-- Using valid SQLite, answer the following questions for the tables provided above.
\\
\\-- How many singers do we have?
\\SELECT \\

==> app_example/ctb_standard_fig.tex <==
% \noindent \textbf{Standard Create Table + Select 3 Prompting}
% \centering
\tiny\texttt{\input{app_example/ctb_standard.tex}
}

\begin{figure}[ht]
    \caption{An example prompt under the standard Create Table + Select 3 prompting for 2-shot on Spider.}
    \label{fig:api_standard}
\end{figure}



% \begin{figure}[ht]\ContinuedFloat
%     \noindent \textbf{Standard Create Table + Select 3 Prompting}
%     % \centering
%     \tiny\texttt{\input{app_example/ctb_standard.tex}
%     }
%     % \fontsize{10}{12}
%     \caption{An example prompt under the standard Create Table + Select 3 prompting for 2-shot on Spider.}
%     \label{fig:api_standard}
% \end{figure}


% \noindent \textbf{Standard Create Table + Select 3 Prompting} 

% \noindent An example prompt under the standard Create Table + Select 3 prompting for 2-shot on Spider. \\


==> error_analysis_v1.tex <==

\subsection{Error Analysis}
\label{sec:analysis}


% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=2.0\columnwidth]{figure/error_case_st.png}
%     \caption{Examples of error types, as made by the codex with \COT promptings.\hs{there are many issues in this figure. see some comments in Figure 1. Caption needs to be rephrased as well.}}
%     \label{fig:chain_of_thought_errors}
%     \vspace{-5pt}
% \end{figure*}


\input{tables/error_analysis.tex}
\input{tables/chain_of_thought_error.tex}

 % all of which were deemed incorrect by the test-suite evaluation. The selected error categories were intended to highlight the most intriguing behaviors that were specific to Codex and which we observed in the errors made.

We investigate the errors of the Codex model using \COT, \LTM, and \QDEMPTB promptings on the Spider dataset. The results are presented in Table~\ref{tb:error_analysis}.
% \hs{why do we put it in Table 10? what are other tables before it?}. \carl{sorry. fixed}  
We randomly sample 50 errors from the \COT prompting results.
% \hs{where is Figure 4?} \carl{fixed}
Following the error analysis described  in~\citet{2022arXiv220400498R}, we focus on three types of errors: semantic incorrect (38 errors), ambiguous correct (3 errors), and invalid SQL (9 errors). 
\hs{did you use exactly the same error names as \cite{2022arXiv220400498R}?} \carl{yes, but we did not list the specific subcategories, such as Shortcuts, GROUP BY Convention, or Argmax, for each error type.}
Semantic incorrect refers to queries that differ in meaning from the gold query and are thus considered incorrect. Ambiguous correct denotes queries that are semantically incorrect but still acceptable as the SQL translation of the given question. An example of this would be a predicted SQL query that selects additional columns. For each error type, we provide detailed definitions in Appendix~\ref{sec:details_on_type_errors}.
\hs{do they have a more formal definition of `acceptable'?} \carl{added more details in the appendix}

% To be more specifically, we consider SELECT Convention, SELECT Extra Columns, and Argmax as Ambiguous correct. 
% An example of this would be a predicted SQL query that selects additional columns. \hs{do they have a more formal definition of `acceptable'?} 


% , as shown in Figure \carl{todo}.



In Table~\ref{tb:error_analysis}, we illustrate that \QDEMPTB prompting effectively addresses a significant proportion of errors in all three categories. One possible reason is that the text-to-SQL parsing is too complex for the model, and that \COT prompting can only deliver superior performance once the LLM exhibits a broad range of semantic comprehension and logical reasoning capabilities that are adequate for the task~\cite{wei2022chain}.  For instance, as shown in Table~\ref{tb:chain_of_thought_error_types}, when presented with the question "How many United Airlines flights go to City 'Aberdeen'?", the model with \COT prompting generates reasoning steps that overlook the "airports" table, which contains destination airport information. Additionally, it selects incorrect columns when joining with the "airline" table, resulting in a semantically incorrect SQL query. On the other hand, we also select an error example from \LTM prompting, where similar errors are observed in intermediate steps due to neglecting to join the "airports" and "airlines" tables. Such errors cannot be corrected in subsequent steps.

% we also select a error example from \LTM prompting. We observed similar errors in the intermediate steps as it neglects to join the airports and airlines tables and such errors cannot be corrected in subsequent steps.

In contrast, \QDEMPTB prompting outperforms other approaches by not instructing the model to generate reasoning steps or intermediate queries, which can often introduce minor errors that negatively impact the model's overall performance. \hs{this and the next paragraph are very repetitive.} \carl{fixed}


==> intro_v3_copy.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure*}[t]
    \centering
    \includegraphics[width=2.1\columnwidth]{figure/baselineerres.png}
    \caption{Different prompting methods with multi-step reasoning for text-to-SQL parsing: (a) \COT, (b) \LTM, and our proposed (c) \QDEMP, and (d) \QDEMPTB. }
    %\nop{ To address issues encountered when utilizing \COT and \LTM prompting methods, we introduce the \QDEMP prompting technique, which is a one-stage question decomposition method. This approach helps to avoid small errors generated in the intermediate steps. Moreover, \QDEMPTB prompting is proposed, which enables the model to reason about tables and their columns, as highlighted in (d), in order to match phases mentioned in sub-questions. \xiang{For the illustration figure, I feel we just need the base model to be wrong but others are fine. The purpose is to demonstrate how \LTM in general could help text2SQL and our proposed methods. Detailed error analysis (Least-to-most wrong and QD correct) could move to later experimental results.}} \hsun{why are you highlighting the green and orange parts? explain them if so. b) is still problematic. Other questions: in the prompt, do you have the exact words `API doc prompting' and `input question'? if not, can we not highlight them but change it to underline, b/c there are too many colored blocks? for the first box, can we add `Given:' on the top and for (a-d) can we say `XX prompting outputs:'}
    \label{fig:intro_pic}
    \vspace{-5pt}
\end{figure*}

%\rc{
Text-to-SQL parsing, the task of translating a natural language question into a SQL query, has found wide applications in building natural language interfaces to databases and thus piqued significant research interest in recent years \citep{wang-etal-2020-rat, deng-etal-2021-structure, yu2021grappa, 2022arXiv220400498R,https://doi.org/10.48550/arxiv.2209.01975,https://doi.org/10.48550/arxiv.2302.08468}.
To develop a text-to-SQL parser, a prevalent approach is to collect labeled data and train a model via supervised learning \citep{shaw-etal-2021-compositional, DBLP:journals/corr/abs-2109-05093}.
While effective, this approach necessitates a considerable amount of training data, which is costly to obtain because annotating SQL queries requires programming expertise.
Consequently, the lack of data hinders real-life applications of state-of-the-art parsers, especially on novel databases and unseen domains \citep{suhr-etal-2020-exploring}.
%}

%\rc{
As an alternative to supervised learning, in-context learning \cite{NEURIPS2020_1457c0d6}, an emergent capability of large language models (LLMs), alleviates the need for large-scale data.
With only a few examples, in-context learning enables LLMs to demonstrate performance comparable to or even better than fully supervised models on many NLP tasks, such as question answering, machine translation, and natural language inference \cite{palm_google, kojima2022large, wei2022chain, wei2022emergent, https://doi.org/10.48550/arxiv.2204.01691}.
When applied to text-to-SQL parsing, in-context learning also shows encouraging results, but it still lags behind supervised approaches \citep{2022arXiv220400498R, chang2023dr, liu2023comprehensive}.
% As a result, although it requires significantly less data, we need to resolve in-context learning's underperformance to replace supervised models in text-to-SQL applications.
%}

%\rc{
We hypothesize that the \carl{under-performance} is because text-to-SQL parsing requires complex, multi-step reasoning.
Even for a seemingly simple question, such as ``What is the ID of Kyle," a model has to ground it to database schemas, infer the relational algebra among schema items, and construct syntactically correct SQL clauses. \carl{Recently, the chain-of-thought (CoT) style promptings~\cite{wei2022chain,2022arXiv220510625Z} were proposed and have shown promising results in enhancing multi-step reasoning capabilities.}
To enhance LLMs' reasoning ability, we systematically explore CoT style prompting for text-to-SQL parsing.
Specifically, we seek to answer two research questions:
% (1) How to design the reasoning step prompts for text-to-SQL parsing?
% (2) Is iteratively prompting LLMs for one reasoning step at a time better than prompting them for all steps in a single pass?
%}
%\xiang{
(1) Which prompting style is better, generating all reasoning steps in a single pass, or iterative prompting and \hs{problem} solving?
(2) \carl{What are the challenges associated with applying existing CoT style reasoning steps for text-to-SQL parsing?}
% What plays the most important role in effective reasoning for text-to-SQL parsing? \hs{this seems too general a question; you might change it to sth specific about `error propagation'}
%}

%\rc{
To address the questions, we adopt two widely used prompting methods for text-to-SQL parsing and propose a novel approach that combines their advantages. \carl{As the first method}, we apply \textit{chain-of-thought prompting} \citep{wei2022chain} by drawing an analogy between its problem-solving process and the execution procedure of a SQL query. 
Referring to the logical execution order of SQL clauses \citep{10.1145/3397481.3450667}, we compose the intermediate execution steps in natural language and prompt LLMs to derive them before generating the SQL query.
% Then 
\carl{As the second method}, we follow \citet{2022arXiv220510625Z} to apply \textit{least-to-most prompting} in two stages: (1) reduction: generate a series of sub-questions from the original question and (2) solving: iteratively translate each sub-question into its corresponding SQL query, with the original question as the last sub-question. \carl{However, in our case study\footnote{we will discuss it in Section~\ref{sec:analysis}}, we find that directly applying chain-of-thought and lease-to-most promptings leads to error propagation issues. Their rationales contain very detailed demonstration-specific information and easier to mislead the reasoning process. Furthermore, the least-to-most prompting technique requires additional computational resources due to the multiple stages of reduction and solving.}



Therefore, we propose a new method called \textit{question-decomposition prompting} (\QDEMP). Similar to chain-of-thought prompting, it generates a sequence of reasoning steps and then the SQL query in one pass. \carl{However, we modify the steps to instruct LLMs to decompose the original complex question, akin to the problem reduction stage in least-to-most prompting.} Also, to help LLMs ground database schemas, we design a variant of question decomposition prompting (\QDEMPTB) by including the table and column names involved in each sub-question.
%}%\hs{
We conduct comprehensive evaluations on two text-to-SQL datasets, Spider~\cite{yu-etal-2018-spider} and Spider Realistic~\cite{deng-etal-2021-structure}. 
Our proposed prompting methods substantially outperform existing prompting ones by 2.4 and \carl{1.5} point absolute gains on the development set of Spider \carl{and Spider Realistic, respectively.} 
% \carl{the first dataset}. 
% \hs{can you talk about the two datasets? it's strange to just mention one?}
%\carl{
This result suggests that \carl{the iterative prompting as in least-to-most prompting  may not be necessary, plus it requires additional computational resources} (\textit{RQ1}).
% , improve LLMs' reasoning ability (\textit{RQ1}). 
\carl{In addition, our analysis shows
the proposed the question decomposition prompting methods, which do not instruct LLMs to generate detailed reasoning steps, reduce the chance of error propagation when generating the reasoning steps.} (\textit{RQ2}).

% , which can negatively impact the model’s
% overall performance that chain-of-thought and least-to-most prompting can lead to error propagation in their detailed reasoning steps. \hs{this should be mentioned earlier} \carl{fixed}.(\textit{RQ2}) \carl{To this end, the proposed the question decomposition prompting methods which do not instruct LLMs to generate detailed reasoning steps.}



% \hs{this should be mentioned earlier} \carl{fixed}.
% We highlight that mitigating error propagation is an important factor in effective reasoning for text-to-SQL parsing (\textit{RQ2}) \carl{To this end, we propose the question decomposition prompting methods which do not instruct LLMs to generate detailed reasoning steps.}
%} 
Finally, we evaluate the robustness of our proposed prompting methods by varying the number, selection, and format of in-context examples and show that they can achieve consistently strong performance across different settings.

% Our proposed prompting methods substantially outperform existing prompting ones by 2.4 point absolute gains on the Spider development set.
% Our error analysis reveals that our proposed prompting methods are effective in reducing the chance of error propagation in reasoning steps, thus leading to better overall accuracy. 
% Finally, we evaluate the robustness of our proposed prompting methods by varying the number, selection, and format of in-context examples and show that they can achieve consistently strong performance across different settings.
%}

==> introdcution.tex <==

\section{Introduction}


\begin{figure*}[t]
    \centering
    \includegraphics[width=2.1\columnwidth, trim={70 0 0 0}]{figure/baselineerres.png}
    \vspace{-2pc}
    \caption{(a) \COT, (b) \LTM, (c) \QDEMP, and (d) \QDEMPTB promptings for the Text-to-SQL parsing. To address issues encountered when utilizing \COT and \LTM prompting methods, we introduce the \QDEMP prompting technique, which is a one-stage question decomposition method. This approach helps to avoid small errors generated in the intermediate steps. Moreover, \QDEMPTB prompting is proposed, which enables the model to reason about tables and their columns, as highlighted in (d), in order to match phases mentioned in sub-questions. \xiang{For the illustration figure, I feel we just need the base model to be wrong but others are fine. The purpose is to demonstrate how \LTM in general could help text2SQL and our proposed methods. Detailed error analysis (Least-to-most wrong and QD correct) could move to later experimental results.} \hs{there are many `small' issues in this figure: `ground true answer', a red curve under `QDecomp', move the `wrong/right' icon to the answer part of the generation rather than besides the name of prompting? These are serious issues that make the paper look far from ready.}}
    \label{fig:intro_pic}
    \vspace{-5pt}
\end{figure*}

% We find \LTM prompting directly may result in error propagation issues where the model finds it challenging to rectify intermediate answers during the solving stage. To address this problem, we suggest using the  \QDEMP prompting, which is a one-stage question decomposition prompting for the Text-to-SQL task. This approach helps to avoid small errors generated in the intermediate steps. Moreover, \QDEMPTB prompting is proposed, which enables the model to reason on tables and their columns that are highlighted to match the phases mentioned in the sub-question. \xiang{For the illustration figure, I feel we just need the base model to be wrong but others are fine. The purpose is to demonstrate how \LTM in general could help text2SQL and our proposed methods. Detailed error analysis (Least-to-most wrong and QD correct) could move to later experimental results.} \hs{there are many `small' issues in this figure: `ground true answer', a red curve under `QDecomp', move the `wrong/right' icon to the answer part of the generation rather than besides the name of prompting? These are serious issues that make the paper look far from ready.
    % \caption{(a) \COT, (b) \LTM, (c) \QDEMP, and (d) \QDEMPTB promptings for the Text-to-SQL task. It is mentioned that using \COT prompting can result in the model failing to identify relevant columns during the reasoning stage. On the other hands, the \LTM prompts directly may result in error propagation issues where the model finds it challenging to rectify intermediate answers during the solving stage. As a solution, we suggest using the \QDEMPTB prompting for Text-to-SQL task. The \QDEMPTB prompts the model to reason on tables and their columns, which are highlighted, to match phases mentioned in the sub-question. \xiang{For the illustration figure, I feel we just need the base model to be wrong but others are fine. The purpose is to demonstrate how \LTM in general could help text2SQL and our proposed methods. Detailed error analysis (Least-to-most wrong and QD correct) could move to later experimental results.} \hs{there are many `small' issues in this figure: `ground true answer', a red curve under `QDecomp', move the `wrong/right' icon to the answer part of the generation rather than besides the name of prompting? These are serious issues that make the paper look far from ready.}}

% compare
% ground truth


% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=2.0\columnwidth]{figure/least-to-most_error.png}
%     \caption{Least-to-Most (left), \textbf{QDecomp} (Middle), and \textbf{QDecomp} + Intermediate Columns prompts for the Text-to-SQL task. It has been noted that utilizing the Least-to-Most prompts directly may result in error propagation issues where the model finds it challenging to rectify intermediate answers during the solving stage. As a solution, we suggest using the \textbf{QDecomp} and \textbf{QDecomp} + Intermediate Columns prompts for Text-to-SQL task. In comparison to the \textbf{QDecomp} prompt, the \textbf{QDecomp} + Intermediate Columns prompt prompts the model to reason on tables and their columns, which are highlighted, to match phases mentioned in the sub-question. \xiang{For the illustration figure, I feel we just need the base model to be wrong but others are fine. The purpose is to demonstrate how least-to-most in general could help text2SQL and our proposed methods. Detailed error analysis (Least-to-most wrong and QD correct) could move to later experimental results.}}
%     \label{fig:intro_pic}
%     \vspace{-5pt}
% \end{figure*}

% These instructions are for authors submitting papers to *ACL conferences using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} and this document contains additional instructions for the \LaTeX{} style files.

% The templates include the \LaTeX{} source of this document (\texttt{acl.tex}),
% the \LaTeX{} style file used to format it (\texttt{acl.sty}),
% an ACL bibliography style (\texttt{acl\_natbib.bst}),
% an example bibliography (\texttt{custom.bib}),
% and the bibliography for the ACL Anthology (\texttt{anthology.bib}).


% 1. while the chain of thought and least-to-most approaches have proven effective in many tasks, it is important to note that the Text-to-SQL task is notably complex. As such, our study focuses on identifying the most effective prompting strategy specifically for this task.


% 2. text2sql may be too complicate so we study how to break down the original query and then further propose to use intermediate columns as guidance.

% 3. Least-to-Most suffers from error propagation.

% The process of converting natural language questions to SQL queries, commonly known as Text-to-SQL, is a \carl{language translation problem}
% \hs{it is not just a business problem; please revise} \carl{fixed}
% that has piqued significant research interest.

\zts{}


\xiang{Text-to-SQL parsing, the process of converting natural language questions to SQL queries, has piqued significant research interest in recent years.}
To accomplish this task, the prevalent approach involves training a model to generate a SQL query by supplying a question, a database schema, and, if necessary, database content as inputs~\cite{shaw-etal-2021-compositional, DBLP:journals/corr/abs-2109-05093}.
While effective, supervised fine-tuning necessitates gathering a considerable amount of data to fine-tune the model, which is costly to obtain for tasks like Text-to-SQL parsing that require domain expertise.
% Moreover, these results are obtained under the assumption that the test data is produced from the same distribution as the training data~\cite{chang2023drspider}.


On the other hand, prompting or in-context learning (ICL), coupled with the recent advancements in large-scale pre-trained language models (LLMs), has demonstrated remarkable flexibility and the ability to perform at or above the level of model fine-tuning in many scenarios~\cite{DBLP:journals/corr/abs-2201-11903, https://doi.org/10.48550/arxiv.2204.02311, wei2022emergent, https://doi.org/10.48550/arxiv.2205.11916, https://doi.org/10.48550/arxiv.2204.01691}.
% \carl{Hence, using LLMs for the Text-to-SQL task offers a promising alternative} to supervised finetuning, requiring only a few examples. \xiang{Directly mention LLM for text2SQL here rather than general in-context learning.}
\xiang{Recent studies have also shown encouraging results in applying in-context learning for Text-to-SQL. However, despite being exposed to numerous SQL queries during pre-training, LLMs still lag behind supervised approaches. One possible explanation is that even the translation of seemingly simple queries, such as "what is the id of Kyle", requires complex, multi-step reasoning to ground the query to DB columns and construct appropriate \texttt{SELECT} and  \texttt{WHERE} clauses.} 
%\carl{do we need to emphasize the hardness of text-to-sql here? since I talk about it again in the following.}

\zts{Two widely adopted methods to enhance the reasoning ability of LLMs and enable them to tackle complex tasks are chain-of-Thought~\cite{DBLP:journals/corr/abs-2201-11903} and Least-to-Most~\cite{https://doi.org/10.48550/arxiv.2205.10625} promptings. These techniques break down complex tasks into a sequence of intermediate steps, eliciting LLMs to gradually derive answers step by step. However, Chain-of-Thought rationales always contain very detailed demonstration-specific information, which is less generalizable to the unseen inference examples and easier to mislead the reasoning process. Although Least-To-Most prompting can generalize better to the examples that are unseen in the prompt than Chain-of-Thought prompting, it requires reducing and multiple solving stages, which takes several times the computational and time costs to call codex API. To address these two issues, we provide one-stage prompting, which only keeps the problem reduction process as the most important hint to elicit reasoning, while removing the problem solving process that contains sub-SQLs for better generalization. \\
% So for prompt design, the rationale is important to ease the burden of the model to generate answers especially for complex tasks. But how to choose the most important hints as the rationales to be both precise, important, and generalizable are important. We take text-to-SQL, a realistic, complex and challenging task as an example, to dig deeper the basic rule of how the prompt can be better for LLMs reasoning. \\
Thus, we propose two strategies for text-to-SQL prompting: QD and QD+Col. QD merges all sub-questions into one stage (save costs) while maintaining the most important task-specific rationale/hints (subquestions) to elicit reasoning. QD+Col further explicitly instructs the model to identify the intermediate tables and columns used to solve each sub-question. These additional reasoning hints enable the model to ground appropriate tables and columns in the questions, providing guidance for generating accurate final SQL queries.}

% The \COT and least-to-most prompting techniques, which have recently emerged, are gaining recognition for their guidance for LLMs to simplify intricate tasks.
\xiang{Two widely adopted methods to enhance the reasoning ability of LLMs and enable them to tackle complex, multi-step tasks are Chain-of-Thought~\cite{DBLP:journals/corr/abs-2201-11903} and Least-to-Most~\cite{https://doi.org/10.48550/arxiv.2205.10625} promptings.}
These techniques break down complex tasks into a sequence of intermediate steps, allowing LLMs to generate answers by using their understanding of semantics and logical reasoning. Consequently, LLMs that use these techniques achieve state-of-the-art performance on a variety of challenging natural language processing tasks. In this regard, this study investigates the potential of adopting such divide-and-conquer ideas to improve the Text-to-SQL parsing capabilities of LLMs.

% 0330 

% Text-to-SQL is a challenging task for LLMs that requires the model to match phrases in the question with columns in the tables and corresponding SQL operations before inferring the join paths between them. In this regard, this study investigates the potential of adopting such divide-and-conquer ideas to improve the Text-to-SQL capabilities of LLMs.



% In this regard, this study investigates the potential of these two prompting techniques, \COT and \LTM, in guiding LLMs to answer the Text-to-SQL task.
% In this regard, this study investigates the potential of adopting such divide-and-conquer ideas to improve the Text-to-SQL capabilities of LLMs.
% \xiang{Elaborate more on the motivation of applying COT/\LTM to text2SQL. And show that it does improve over the baseline.}


However, our attempts to directly apply these techniques to the Text-to-SQL parsing have encountered difficulties. Specifically, the \COT prompting approach struggles when attempting to solve complex tasks, as the large language models (LLMs) lack sufficient in-context learning exemplars to learn all the necessary reasoning steps, as cited in~\cite{https://doi.org/10.48550/arxiv.2210.02406}. Consequently, LLMs cannot acquire adequate semantic understanding and logical reasoning skills to answer questions, as noted in~\cite{https://doi.org/10.48550/arxiv.2201.11903}. For example, the demonstrations for generating a complex SQL query with multiple conditional clauses, including \texttt{WHERE}, \texttt{JOIN}, \texttt{GROUP BY}, and \texttt{ORDER BY} clauses, are inadequate for the Codex to learn how to answer similar questions that require multiple conditional clauses to satisfy conditions. Additionally, we have identified that the \LTM prompting approach may suffer from the error propagation issue on the Text-to-SQL parsing. That is, LLMs generate intermediate answers that may contain errors, which cannot be corrected during the solving stage\footnote{We will discuss these in Section~\ref{sec:analysis}} 


% \carl{I don't talk about issue of Least-to-most very clearly. Besides, I leave the error analysis in the later section. is it ok?}



% However, we have discovered challenges in directly applying these techniques to the Task-to-SQL task. Specifically, the \COT prompting, which is known to struggle with complex tasks when LLMs lacks sufficient demonstrations for current models to learn all necessary reasoning steps~\cite{https://doi.org/10.48550/arxiv.2210.02406} and thus can't demonstrate enough semantic understanding and logical reasoning~\cite{https://doi.org/10.48550/arxiv.2201.11903} for the given question. For example, few demonstrations of generating a complicated SQL query with multiple different conditional clauses, including where, join, group by, and order by clauses, are insufficient for Codex to learn how to answer similar questions that also require multiple conditional clauses to meet conditions. In addition, we identifies that the \LTM prompting may suffer from the error propagation issue on the Task-to-SQL task. That is, it makes errors in generating the intermediate answer and can't correct it in the solving stage. In other words, it is challenging for Codex to correct intermediate answers during the solving stage, as shown in Figure~\ref{fig:intro_pic}.



% The recent proposed two promptings, namely Chain-of and \LTM, are well known good at decomposing the complex tasks into series of intermediate steps and elicits reasoning in large language models and thus outperforms the state-of-the-art results on many challenging natural language processing tasks, such as Text-to-SQL task.  To answer the sql query for a given question, the model needs to first match the phase in the question with column in the tables and the corresponding sql operations. Then, the model need to infer join paths between the matched columns and selected sql operations. It make challenging for the model. Thus, in this study, we explore the potential of two recently proposed prompting techniques, namely Chain-of and \LTM, in guiding the prediction of large language models on the Text-to-SQL task.



% , as tasks become more complex, few demonstrations of the complex
% task aren’t sufficient for current models to learn to perform all necessary reasoning steps. E.g., fewshot demonstrations of concatenating the kth letter of words in a string is insufficient for GPT-3 to learn to extract the k
% th letter, or learn to answer hard single-hop questions when only provided a few demonstrations of multi-hop questions


To address these issues, we propose two novel question decomposition prompting \xiang{strategies}: \QDEMP and~\QDEMPTB. First, \QDEMP prompting is a one-stage approach that addresses the error propagation issue identified in the \LTM prompting.  The model focuses on decomposing the original question without generating intermediate answers for sub-questions, followed by generating the final SQL query. This reduces the likelihood of errors being made. Second, we draw inspiration from a recent study by~\citet{2022arXiv220510625Z}
that emphasizes the importance of identifying tables and columns in each step to improve phrase matching with relevant tables and columns. Thus, we propose~\QDEMPTB prompting, where the model is instructed to identify the intermediate tables and columns used to solve each sub-question. This additional reasoning step enables the model to better match phrases with the appropriate tables and columns, providing guidance for generating accurate final SQL queries.


% \hs{there should be no bracket outside a citation when it plays a role in the sentence. use ``~\citet{2022arXiv220510625Z}''} \carl{fixed} 

We provide empirical evaluations on various Text-to-SQL databases, including Spider and Spider Realistic. Our proposed prompting techniques outperform other prompting methods. 
We also conduct an error analysis, which reveals that the proposed prompting approach is effective in addressing a considerable portion of errors. Furthermore, the robustness experiments demonstrate that the proposed promptings sustain competitive performance even when we vary the number and selection of exemplars and the prompting format.

% TOs 
% chatgpt price regular gpt4. pay service cheaper than gpt4. Time time run few times. pick some experimnets. ablation study. 

% standard baseline, how many runs. 10 runs for single setting. two round. best, medium performance. don't worry chatgpt now. best effort I can. whelther we need to run gpt3. disturbance. plan. may not be needed. more  convince to chatgpt. budget. ablation study. which setting is meaningful. 

% too costly. comprehensively. result. be firm and push back. focus on writing part. annoying part. best effort. do a pass. most meaning ablation setting. 

% think hard on how to better revise. think better. improve your writing. give me a version can't do any better. 

% other dataset. codex has stopped. re-run all. selection operations. \
% still add this result. how we got them. select clauses. correct prompt 5 dataset. 
% add the result first to the appendix. select column. full column name. 

% run openapi tokenizer. one spider input and output. estimate the cost for each prompting 

% focus on paper writing. bandwith. put a version on arxiv. fresh. anymore. 












% We provide empirical evaluations on various Text-to-SQL databases, including Spider and Spider Realistic. Our proposed prompting techniques outperform other promptings, as demonstrated by the results of the evaluations.  We analyze the predicted queries that automatic evaluation judged as wrong and find that the proposed prompting addresses a significant proportion of errors. Besides, the robustness experiments shows that the proposed prompting can achieve better performance even when we vary number of exemplars, choice of exemplars, prompting format.


% \carl{todo}

% our methods beyond the training domains.
% We present empirical evaluations on different Text-to-SQL databases, such as Spider, GeoQuery, and Scholar. It shows that compared to other baselines, our proposed promptings methods achieve best performance. Besides, we have condocuted cross-domain generalization experiment. 



% To address these, we further propose \textbf{QDecomp} and \textbf{QDecomp + Intermediate Columns}, First, for QDecomp, it is a one-stage approach. To avoid error propagation issue identified in \LTM prompting. The model is asked focus on decomposing the original question without generate the answers for sub-questions, followed by generating the final SQL query. Second, inspired by~\cite{2022arXiv220510625Z}, which highlights tables and columns in each step to better match the phrases with the relevant tables and columns, we further proposes \textbf{QDecomp + Intermediate Columns}, in which the model is asked to identify the intermediate tables and columns for solving each sub-question. 



% Figure 2 illustrates one such result—on the GSM8K benchmark of math word problems
% (Cobbe et al., 2021), \COT prompting with PaLM 540B outperforms standard prompting
% by a large margin and achieves new state-of-the-art performance. A prompting only approach is
% important because it does not require a large training dataset and because a single model checkpoint can perform many tasks without loss of generality. This work underscores how large language models
% can learn via a few examples with natural language data about the task (c.f. automatically learning
% the patterns underlying inputs and outputs via a large training dataset).



% while the chain of thought and \LTM approaches have proven effective in many tasks, it is important to note that the Text-to-SQL task is notably complex. As such, our study focuses on identifying the most effective prompting strategy specifically for this task.

% study if such models are already competitive Text-to-SQL solutions without any further
% finetuning on task-specific training data, evaluating
% Codex and GPT-3 models of different sizes with
% varied prompts on Text-to-SQL benchmarks



% Translating natural language questions to SQL
% queries (Text-to-SQL) is an important business
% problem which has seen significant research interest. A common approach to this task involves training a model to produce a SQL query when given a question, a database schema, and possibly database content as inputs. Although effective, supervised finetuning requires to collect significant amount of data to finetune  the model. In addition, those results are obtained in the setting where test data are created with the same distribution as training data~\cite{chang2023drspider}. On the other hands, Prompting is sufficiently flexible
% and, with recent advancement of large-scale pretrained language models (LLMs), able to  perform on-par or better than model finetuning in many cases~\cite{DBLP:journals/corr/abs-2201-11903, https://doi.org/10.48550/arxiv.2204.02311, wei2022emergent, https://doi.org/10.48550/arxiv.2205.11916, https://doi.org/10.48550/arxiv.2204.01691} This new, few-shot learning paradigm is called in-context learning and has become an attractive alternative to supervised finetuning.

% has become an
% effective and generic approach to address a wide range of language understanding problems. B


% Large language models can perform downstream tasks by conditioning generation given promptings 


% on a few task demonstrations, thereby avoiding the need for data collection and any parameter updates. This new, few-shot learning paradigm is called in-context learning and has become an attractive alternative to supervised finetuning


% Results from the broader field demonstrate that
% Large language models can perform in-context learning with different prompting approaches, where they learn a new task from a few task demonstrations, without any parameter updates. It has become an attractive alternative to supervised finetuning.



% Large language models can perform downstream tasks by conditioning generation on a few task demonstrations, thereby avoiding the need for any parameter updates. This new, few-shot learning paradigm is called in-context learning and has become an attractive alternative to supervised finetuning

% simply scaling training data and model size for generative language models brings advanced capabilities, such as few-shot learning without finetuning (GPT-3, Brown et al., 2020) and
% code generation (Codex, Chen et al., 2021).


% Recent proposed prompting approaches, such as \COT and \LTM promptings allows 


% narrowing the gap between human intelligence and machine intelligence.


% results from the broader field demonstrate that simply scaling training data and model size for generative language models brings advanced capabilities, such as few-shot learning without finetuning (GPT-3, Brown et al., 2020) and
% code generation (Codex, Chen et al., 2021). In
% this work we study if such models are already competitive Text-to-SQL solutions without any further finetuning on task-specific training data, evaluating Codex and GPT-3 models of different sizes with varied prompts on Text-to-SQL benchmarks.



% A clear trend in this area is to finetune models pretrained on natural language; notably, performance significantly improves as larger pretrained models are used (Shaw et al.,
% 2021; Scholak et al., 2021).

% Recent results from the broader field demonstrate that simply scaling training data and model size for generative language models brings advanced capabilities, such as few-shot learning without finetuning (GPT-3, Brown et al., 2020) and
% code generation (Codex, Chen et al., 2021). In
% this work we study if such models are already competitive Text-to-SQL solutions without any further
% finetuning on task-specific training data, evaluating
% Codex and GPT-3 models of different sizes with
% varied prompts on Text-to-SQL benchmarks

==> introduction_v2.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure*}[t]
    \centering
    \includegraphics[width=2.1\columnwidth]{figure/baselineerres.png}
    \caption{Different prompting methods with multi-step reasoning for text-to-SQL: (a) \COT, (b) \LTM, and our proposed (c) \QDEMP, and (d) \QDEMPTB.\nop{ To address issues encountered when utilizing \COT and \LTM prompting methods, we introduce the \QDEMP prompting technique, which is a one-stage question decomposition method. This approach helps to avoid small errors generated in the intermediate steps. Moreover, \QDEMPTB prompting is proposed, which enables the model to reason about tables and their columns, as highlighted in (d), in order to match phases mentioned in sub-questions. \xiang{For the illustration figure, I feel we just need the base model to be wrong but others are fine. The purpose is to demonstrate how \LTM in general could help text2SQL and our proposed methods. Detailed error analysis (Least-to-most wrong and QD correct) could move to later experimental results.}} \hsun{why are you highlighting the green and orange parts? explain them if so. b) is still problematic. Other questions: in the prompt, do you have the exact words `API doc prompting' and `input question'? if not, can we not highlight them but change it to underline, b/c there are too many colored blocks? for the first box, can we add `Given:' on the top and for (a-d) can we say `XX prompting outputs:'}}
    \label{fig:intro_pic}
    \vspace{-5pt}
\end{figure*}

\hs{text-to-SQL parsing, the task of converting natural language question to SQL query, has piqued significant research interest in recent years \cite{wang-etal-2020-rat, yu2021grappa, deng-etal-2021-structure,2022arXiv220400498R,https://doi.org/10.48550/arxiv.2209.01975,https://doi.org/10.48550/arxiv.2302.08468}.
To accomplish this task, one prevalent approach is to train a model that takes a question, a database (DB) schema, and (optional) DB content as input and outputs a SQL query ~\cite{shaw-etal-2021-compositional, DBLP:journals/corr/abs-2109-05093}.
While effective, such approaches necessitate a considerable amount of training data, which is costly to obtain, since annotating SQL queries requires domain expertise.}
% Moreover, these results are obtained under the assumption that the test data is produced from the same distribution as the training data~\cite{chang2023drspider}.

\hs{On the other hand, in-context learning (ICL) \cite{NEURIPS2020_1457c0d6}, an emergent capability of large language models (LLMs), has demonstrated remarkable performance that is comparable to or even better than fully supervised models \carl{for many tasks~\cite{wei2022chain, palm_google, wei2022emergent, kojima2022large, https://doi.org/10.48550/arxiv.2204.01691}, such as question answering, machine translation and NLI.}
% \hsun{here what do we mean by `in many scenarios'? are we talking about text-to-sql only or many tasks? change it to `for many tasks such as XYZ'? The last two references starting with `https' seem very strange.}.
% \carl{Hence, using LLMs for the text-to-SQL task offers a promising alternative} to supervised finetuning, requiring only a few examples. \xiang{Directly mention LLM for text2SQL here rather than general in-context learning.}
Recent studies \cite{2022arXiv220400498R,liu2023comprehensive, chang2023dr} have also shown encouraging results when applying in-context learning to text-to-SQL parsing. However, despite being exposed to numerous SQL queries during pre-training, LLMs still lag behind supervised approaches \hs{\cite{2022arXiv220400498R,liu2023comprehensive}}. One possible explanation is that even the translation of seemingly simple queries, such as ``what is the id of Kyle'', requires complex, multi-step reasoning in order to ground the query to DB columns and construct appropriate \texttt{SELECT} and  \texttt{WHERE} clauses.} 
%\carl{do we need to emphasize the hardness of text-to-sql here? since I talk about it again in the following.}

\hs{Two widely adopted methods to enhance the multi-step reasoning ability of LLMs and enable them to tackle complex tasks are chain-of-thought~\cite{wei2022chain} and least-to-most prompting~\cite{2022arXiv220510625Z}.\nop{With a few demonstration examples that decompose a complex task into a sequence of intermediate steps,} Chain-of-Thought (CoT) prompts an LLM to derive a sequence of intermediate steps before arriving at the final answer.} \hsun{DESCRIBE how least-to-most prompting works in general.} 

\hsun{Gist of this paragraph: Inspired by the above two methods, this paper explores CoT style prompting for text-to-SQL. To apply CoT to text-to-SQL, we DID WHAT...(note that it is not so straightforward why we formulate the reasoning chains this way. you should mention the execution order of SQL, i.e., essentially following the intrinsic process of how SQL is executed like the math problem solving process, using templates from previous paper, even with just a few sentences.) To apply least-to-most, we DID WHAT... (refer to Figure 1.) In this paper, we seek to answer two research questions: (1) which kind of reasoning steps are better? (2) one-stage or iterative? Towards that, we design a new prompting method, XX, which [how it works]. Moreover, we propose another variant of XX by including table/column names incrementally involved in each step, where the intuition is that ...} 

\hs{--probably will remove the following two paragraphs--}

\hs{[probably rephrase sth and remove the rest:]}\zts{However, Chain-of-Thought rationales always contain very detailed demonstration-specific information, which is less generalizable to the unseen inference examples and easier to mislead the reasoning process.\hs{see, if you directly say this, people likely won't buy your arguments, as they don't know what you are talking about or such arguments are not widely accepted/presented yet.} Although Least-To-Most prompting can generalize better\hs{where do we get this conclusion? from the original paper? I feel we shouldn't call it `generalize' anyway, as there is no "working well on training but does not generalize well to testing set" kind of thing in this setting.} to the examples that are unseen in the prompt than Chain-of-Thought prompting, \hs{this is very weird wording and how could you suddenly mention codex API (it's never mentioned earlier): it requires reducing and multiple solving stages, which takes several times the computational and time costs to call codex API}. To address these two issues, we provide one-stage prompting, which only keeps the problem reduction process as the most important hint to elicit reasoning, while removing the problem solving process that contains sub-SQLs for better generalization. \hs{People probably don't know what you are talking about, even if they have read the above two papers, not to mention for people who haven't.. You have created Figure 1, but why not refer to it in Intro??}\\
% So for prompt design, the rationale is important to ease the burden of the model to generate answers especially for complex tasks. But how to choose the most important hints as the rationales to be both precise, important, and generalizable are important. We take text-to-SQL, a realistic, complex and challenging task as an example, to dig deeper the basic rule of how the prompt can be better for LLMs reasoning. \\
\hs{[probably rephrase sth and remove the rest:]} Thus, we propose two strategies for text-to-SQL prompting: QD and QD+Col. QD merges all sub-questions into one stage (save costs) while maintaining the most important task-specific rationale/hints (subquestions) to elicit reasoning. QD+Col further explicitly instructs the model to identify the intermediate tables and columns used to solve each sub-question. These additional reasoning hints enable the model to ground appropriate tables and columns in the questions, providing guidance for generating accurate final SQL queries.}


\hs{We conduct comprehensive evaluations on various text-to-SQL databasets, including Spider~\cite{yu-etal-2018-spider}, Spider Realistic~\cite{deng-etal-2021-structure}, and XYZ. Our proposed prompting methods substantially outperform existing prompting ones by XX point absolute gains. \carl{todo}
Our error analysis reveals that our proposed prompting methods are effective in addressing a considerable portion of errors \hsun{say sth more informative, e.g., which category of errors has been most significantly reduced?} \carl{todo}. Furthermore, we evaluate the robustness of our proposed prompting methods by varying the number and selection of exemplars as well as the prompt format and show that they can achieve consistently strong performance across different settings.}
\nop{We provide empirical evaluations on various text-to-SQL databases, including Spider and Spider Realistic. Our proposed prompting techniques outperform other prompting methods. 
We also conduct an error analysis, which reveals that the proposed prompting approach is effective in addressing a considerable portion of errors. Furthermore, the robustness experiments demonstrate that the proposed promptings sustain competitive performance even when we vary the number and selection of exemplars and the prompting format.}


==> method.tex <==
\section{Prompting for Multi-Step Reasoning in Text-to-SQL}
\label{sec:promptdesgin}

% In this section, we provide additional details on how to design prompts based on the principles of each prompting technique for the text-to-SQL task. 
%\xiang{In this section, we describe our prompting strategies to decompose the original natural language question and guide the LLM to progressively construct the target SQL query.}
\hs{In this section, we describe several prompting strategies to guide an LLM to derive a sequence of reasoning steps that lead to the target SQL query progressively.}
\xiang{We first describe how we adapt Chain-of-Thought and Least-to-Most prompting to the task of text-to-SQL parsing.}
% \hs{do we need to keep the names capitalized? double check the convention.}
\carl{todo} %We then introduce two new prompting strategies we designed to better} \carl{avoid errors generated by the model in intermediate steps}
\hs{To address the two research questions mentioned in Section \ref{sec:intro}, we introduce two new prompting strategies: \QDEMP and \QDEMPTB.}
\hs{Figure \ref{fig:intro_pic} demonstrates different prompting methods and more examples are provided in Appendix \ref{sec:app_prompt_format}.}
\nop{
More examples of prompting are provided in the Appendix~\ref{sec:app_prompt_format}}


\hsun{should we mention here we used Codex for our experiments, before OpenAI discontinued its API support?}
% For each prompting, we have more examples shown in appendix~\carl{todo}.

\carl{In this work, we mainly use Codex (code-davinci-002)~\cite{DBLP:journals/corr/abs-2107-03374} 
% \hs{do we need to specify version, time-range, or anything for transparency or reproducibility?} \carl{fixed} 
hosted by OpenAI as the LLM for all experiments described in this paper.
% Codex is trained on a diverse set of sources from the internet and further fine-tuned on code from GitHub.
\hs{Greedy decoding with temperature 0 is used for generation}. The experiments were conducted between January and March 2023 through OpenAI API~\footnote{\url{https://openai.com/api/}}.}

\hsun{this part is OK, but make sure you didn't mention Codex before this, otherwise, maybe move this to the beginning paragraphs of Section 3.}
\carl{fixed}


%\rc{I think for this paper, it might be better to first discuss related work to explain CoT and \LTM clearly. Then, this section will just (1) briefly discuss how we construct two baselines and (2) focus on describing our QD prompting}

% \input{tables/chainofthoughtprompt.tex}
%  

\subsection{\COT prompting}
\label{sec:chain_of_though_prompt_design}

% \textbf{COT} asks \hs{the} model to generate a sequence or chain of intermediate reasoning steps and then derive the final SQL query based on those steps. Here, we follow \hs{the} order of steps outlined in~\cite{10.1145/3397481.3450667} to generate the intermediate reasoning steps for each in-context exemplar.
% \xiang{Xiang: Let's make these two sections shorter, these are more like our baselines. Emphasis more on how our implementation is similar to what was used in the original paper.}
% \xiang{Describing the strategies progressively. A short description of \COT and potential issues with it in our setting. A slightly more detailed description for \LTM and a detailed description of our method.}

\xiang{Chain-of-Thought prompting aims to} generate a coherent series of intermediate reasoning steps before predicting the final answer. % and has been shown to enhance the reasoning capabilities of language models. of a chain-of-thought prompt for the text-to-SQL task
\xiang{For text-to-SQL parsing, the underlying reasoning steps are essentially the SQL operations and clauses that collectively construct the final query. Therefore, we design our Chain-of-Thought as describing the logical execution process of the SQL query, similar to~\citet{10.1145/3397481.3450667}. An example is shown in}\carl{ Figure~\ref{fig:intro_pic}(a)}.
% An example is provided in Table~\ref{tb:chain_of_thought}, which follows the steps outlined in~\cite{10.1145/3397481.3450667} to design the intermediate reasoning steps for each in-context exemplar. 
%Specifically, the sequence of reasoning steps are generated according to the logic execution order defined for the SQL operations.
%, including the \texttt{FORM}, \texttt{JOIN}, \texttt{WHERE}, and \texttt{GROUP BY} clauses. 
% For instance, when given the question "Find papers whose second author has last name 'Turon' and is affiliated with an institution in the country 'USA'," the first reasoning step would involve focusing on the \texttt{FROM} and \texttt{JOIN} clauses.
%to identify the tables that contain the relevant data. 
% Next, the \texttt{Where} constraints are used to filter out any irrelevant data. Finally, the \texttt{SELECT} clause is employed in the last reasoning step to output the appropriate columns for answering the question. 
However, it is important to note that the model's ability to generate these detailed reasoning steps depends on its semantic comprehension and logical reasoning capabilities, which if inadequate, may result in decreased performance~\cite{wei2022chain}. \hs{is the last sentence informative? does it not apply to every model? I kind of feel it is obvious.}

% 03/26



% Table \carl{todo} shows an example of a \COT prompt for the text-to-SQL task.  Here, we follow \hs{the} order of steps outlined in~\cite{10.1145/3397481.3450667} to design the intermediate reasoning steps for each in-context exemplar. In more details, it follow the logical order of a SQL operations, such as FORM, JOIN, WHERE, and GROUP BY clauses, when generating the sequence of reasoning steps. Given question "Find papers whose second author has last name 'Turon' and is affiliated with an institution in the country 'USA'.", the first reasoning step focus on "FROM" and "JOIN" clauses to find the tables to determine the working set of data. Next "Where" constrains are applied to filter the data the do not satisfy the constrain. In the last reasoning step, "SELECT" clause is used to output the columns for answering the question.





% It first categorizes the query, then generates
% quasi-alignments between the text and output statements. This represents synchronicity in the same spirit as other higher performing semantic parsers do (Qiu et al., 2022a), but the intermediate constituents and clauses need not map exactly to what is seen in the input and output. The flexibility of \COT is convenient for data like CFQ where inclusion of variables is not compatible with synchronous grammar training and inference (Wong & Mooney, 2007).


\subsection{\LTM prompting}
\LTM Prompting~\cite{2022arXiv220510625Z} tackles complex questions by breaking them down into a series of sub-questions with increasing levels of difficulty. It consists of two stages: question decomposition and solving \hs{did the paper use exactly the same wording? double check}. \carl{they use 1. problem reduction 2. problem solving} During the question decomposition stage, the LLM decomposes the original question into a set of easier sub-questions.
\xiang{During the solving stage, the LLM takes in the sub-questions one at a time, and gradually builds up the final solution. \hs{`gradually' does not seem the most precise word; can we use `iteratively'? (also to echo our second research question?)} This differs from Chain-of-Thought prompting, where the LLM is instructed to generate all the reasoning steps altogether.}
% To achieve this, the model is provided with examples that demonstrate the decomposition, followed by a specific question to be reduced. In the solving stage, the model generates SQL queries for each sub-question identified in the first stage.
% The Appendix \carl{todo} contains example prompts for both stages.
% Examples taken from the \LTM prompt in both stages are presented in Table~\ref{tb:least_to_most_promoting}.

\xiang{For question decomposition, we supply in-context examples that divide the original question into segments using conjunction words (such as "and," "or", and "but") or prepositions (such as "with" and "without") to produce sub-questions. }
% To generate the set of easier sub-questions for text-to-SQL parsing, we follow the existing work~\cite{DBLP:journals/corr/abs-2112-06311}, where they consider it is easier for the model to concentrate on a subset of SQL clauses when solving each sub-question.
% Thus, during the sub-question annotation process, we divide the original question into segments using conjunction words (such as "and," "or", and "but") or prepositions (such as "with" and "without") to produce sub-questions. 
This segmentation allows the model to focus on only a subset of SQL clauses for each sub-question, thereby decreasing the complexity of the original problem~\cite{DBLP:journals/corr/abs-2112-06311}.
\xiang{After decomposition, the LLM then generates the partial query associated with each sub-question and outputs the complete SQL query in the end.}
For instance, given the question "Show first name, last name, age for all female students. Their sex is F.", shown in Figure~\ref{fig:intro_pic}(b), the sub-problems are "Show first name, last name, age for all students." and "Show first name, last name, age for all female students." For the first sub-question, the model can focus on constructing the \texttt{SELECT} and \texttt{FROM} clauses, while for the remaining question, the model can focus solely on the \texttt{WHERE} clause.



% problems are "Find the number of employees hired in each shop." and "Find the number of employees hired in each shop; show the shop name as well.". For the first sub-question, the model can focus on using \texttt{SELECT}, \texttt{FROM}, \texttt{JOIN} and \texttt{GROUP BY} clauses, while for the remaining question, the model can focus solely on \texttt{SELECT} and \texttt{FROM} clauses



% For instance, given the question "What are the names of the stations which serve both Ananthapuri Express and Guruvayur Express trains?", shown in Figure~\ref{fig:intro_pic}, the sub-problems are "What are the names of the stations?" and "What are the names of the stations which serve Ananthapuri Express trains?" For the first sub-question, the model can focus on using \texttt{SELECT} and \texttt{FROM} clauses, while for the remaining question, the model can focus solely on conditional clauses such as \texttt{WHERE} and \texttt{JOIN}.


 \subsection{Question decomposition prompting}

% \input{tables/QDecomp_table.tex}

\st{We have observed that directly adopting \LTM prompting for text-to-SQL parsing can result in sub-optimal performance due to potential errors in intermediate steps. % , as detailed in Section~\ref{sec:results}. 
To address this issue, we study a one-stage question decomposition prompting, called~\QDEMP.} \hs{Given how chain-of-thought and least-to-most prompting work as described above, we are motivated to investigate two research questions: (1)... (2).... To answer these questions, we propose a new prompting method named \QDEMP:
% \hs{can we use a special font for our proposed method? like `texttt'?} \carl{updated texttt version}
Unlike the least-to-most prompting that generates intermediate SQL queries,
the LLM is instructed to focus solely on decomposing the original question first, followed by directly generating the final SQL query based on the simpler sub-questions. A prompting example is shown in Figure~\ref{fig:intro_pic}(c).}

% in Appendix~\ref{sec:app_prompt_format}.

\xiang{Motivated by the importance of matching phrases with relevant tables and columns~\cite{DBLP:journals/corr/abs-2112-06311}\hs{this is not clear; do you want to describe what this paper is doing? how you are motivated?}, we then propose a \st{fine-grained} variant of \QDEMP:}
% \QDEMPTB is a fine-grained variant of the~\QDEMP. 
% Drawing inspiration from \citet{wolfson-etal-2022-weakly}, this work highlights tables and columns that would be used in each step to better match the phrases with the relevant tables and columns.
\xiang{\st{Instead of generating the partial SQL queries,} The LLM is asked to further identify the intermediate\st{tables and columns} \hs{table/column names} for addressing each sub-question (\QDEMPTB)}, as illustrated in Figure~\ref{fig:intro_pic}(d).
% Thus, we propose~\QDEMPTB, which asks the model to identify the intermediate tables and columns for solving each sub-question, as illustrated in Table~\ref{tb:qdecomp_intermediate_table}. 

\hs{To clarify the principle for identifying the ground-truth intermediate tables and columns in \QDEMPTB, let us consider three common scenarios: }
% Next, we will explain how to annotate intermediate tables for the in-context learning set. We have identified three common scenarios in the Spider dataset.
Firstly, when the current sub-question involves column selection operations, such as \texttt{SELECT} and \texttt{FROM} clauses, we will highlight the relevant table-column pairs. Additionally, If there are conditional operations, such as \texttt{WHERE}, \texttt{GROUP BY}, and \texttt{ORDER BY}, we will also highlight the relevant table-column pairs. If the current sub-question involves \texttt{COUNT(*)}, we will substitute it with any column from the table within the sub-query. Secondly, if the \texttt{JOIN} clause is required to satisfy the semantic requirements of the current sub-question, we will highlight table-column pairs for the joining operation. However, we will skip tables that have already been highlighted in prior sub-questions, as an excessive amount of information may cause the model to become confused and diminish its performance, as discussed in Section~\ref{sec:chain_of_though_prompt_design}. Thirdly, if table-column pairs have already been annotated in prior sub-questions, we will skip them and only include the necessary pairs. In situations where no relevant table-column pairs exist in the current step, we will choose one highlighted pair from prior steps to ensure that the model highlights at least one pair in each step. For the purpose of reproducibility, we provided our annotation code online\footnote{\hs{https://github/XX}}.

 % to avoid overwhelming the model with redundant information.

% To provide a concrete example, 
Here, we give a concrete example, as shown in Figure~\ref{fig:intro_pic}(d). Given the sub-question "Show first name, last name, age for all students", the model is instructed to highlight the intermediate table "student" and its columns "fname", "lname" and "age", which are used in conjunction with the \texttt{SELECT} and \texttt{FROM} clauses to solve the sub-question. Subsequently, for the follow-up sub-question "Show first name, last name, age for all female students. Their sex is F", the model is instructed to highlight the intermediate table "student" and its column "sex", which are used together with the conditional clause (i.e., \texttt{WHERE}) to solve the sub-question.


% \carl{todo fix figure}

% Then, we are going to tell how to annotate the intermediate tables for the in-context learning set. We find that there are typically four different cases on the Spider dataset. First, for the current sub-question, the model should focus on the column selection operations, such as \texttt{SELECT} and \texttt{FROM} clauses. We will highlight the tables and their columns for the current sub question. Besides, when the model should focus on the column conditional operations, such as \texttt{WHERE}, \texttt{GROUP BY}, \texttt{ORDER BY}, similar to the previous case, we will highlight the tables and their columns involving operations. Note that if COUNT(*) should be involving the current sub question, we will replace it the any column of table involving in the current subquestion. Second, when the model need to join tables to meet the semantic of current sub-question, we will highlight the table and column should be used for connection. However, we would not include the tables which are already annotate in previous subquestion. The reason is that for the subquestion, it may need to highlight too many table-column pairs and too much detailed information may mislead the model, resulted in decreased performance. Third, if the table-column pairs are already annotated in previous sub-question, we will skip it, keeping the necessary table-column pairs to prevent the too much details information. Note the if there is no table-column pair involving in current step, we will select one table-column pair highlighted in the previous sub-question to avoid the model not highlighting any table-column pair in each step. For the reproducity, we provide our the annotation code.


% ~\carl{A little more details todo}





% make the model focus on 


% we find the current sub-question  is selection operation. Second is condition operations such as  . Third is join path inference.


==> related_work.tex <==
\section{Related work}

\subsection{Few-shot Promptings with LLMs}

% Large-scale Language models (LLMs) have been
% shown to learn various NLP tasks given just few examples as prompts~\cite{NEURIPS2020_1457c0d6}.
 % Recently, researchers start to propose different prompting methods to empower LLMs to perform complex reasoning tasks.

Researchers have been experimenting with just a few examples as prompts~\cite{NEURIPS2020_1457c0d6}, to help large-scale language models (LLMs) perform complex reasoning tasks. One such method is Chain-of-Thought (COT)~\cite{DBLP:journals/corr/abs-2201-11903} which involves providing the intermediate steps needed to arrive at the answer for multi-step reasoning tasks. Another method is least-to-most prompting~\cite{https://doi.org/10.48550/arxiv.2205.10625} which involves 1) breaking down a complex problem into smaller subproblems and 2) solving them in a specific order, using the answers from previously solved subproblems to guide the solution of the next subproblem. Due to the success of these methods in LLMs, many subsequent studies have been proposed in the literature~\cite{kojima2022large, 2022arXiv220308383W, 2022arXiv221003057S, Chen2022LargeLM, Prystawski2022PsychologicallyinformedCP, https://doi.org/10.48550/arxiv.2209.15003, yang-etal-2022-seqzero, https://doi.org/10.48550/arxiv.2210.02406, https://doi.org/10.48550/arxiv.2212.04092}.


However, current research in large language models primarily focuses on text-based tasks such as question answering and common sense reasoning. However, their ability to solve Text-to-SQL tasks, which are considered challenging as they require an understanding of both the question and the underlying table structure to generate a valid SQL query, remains untested.


% two steps: decomposing the complex problem into subproblems and solving these subproblems in a specific order, with each subproblem being facilitated by the answers obtained from previously solved subproblems.

% has been applied to various multi-step reasoning tasks by providing the intermediate reasoning steps needed to arrive at the answer.

% However, current research in large language models primarily focuses on text-based tasks such as question answering and common sense reasoning. However, their ability to solve Text-to-SQL tasks, which are considered challenging as they require understanding of both the question and the underlying table structure to generate a valid SQL query, remains untested.


% the current studies are still heavily
% focused on text-based tasks like question answering, common sense reasoning, etc. However, the models’
% capability to solve Text-to-SQL tasks, which is considered difficult since it not only requires model to understand question but also need to reason table schemes and find corresponding operations to generate valid SQL query, is yet unknown.


% For the Text-to-SQL tasks, which is consider to be more hard , the models’
% capability to solve complex \carl{more details} Text-to-SQL tasks is yet unknown.





% where one prompt is used to generate the sub-questions needed to answer a complex question and
% a second prompt sequentially answers these sub-questions. It consists of two steps:



% needed to arrive at the answer. Building of the successes of Chain-of-thought (CoT) style prompting on LLMs, many subsequent studies have focused on improvements of this basic model. This
% includes, for example, diverse decoding and ensembling to improve self-consistency


% , more complex and contrasting rationales (Marasovic et al., 2021; Wang et al., 2022a), gener- ´
% ating sub-questions and answering them sequentially in least-to-most complexity order (Zhou et al.,
% 2022), integration with symbolic modules (Jung et al., 2022), selection inference (Creswell et al.,
% 2022), coupling in-context learning with sparse fine-tuning (Zelikman et al., 2022), and even presented many of them under a single probabilistic programming framework (Dohan et al., 2022).


% We view these prior works as specialized systems with a pre-defined decomposition structure. For
% example, the closest work to our approach is the idea of least-to-most prompting (Zhou et al., 2022)
% where one prompt is used to generate the sub-questions needed to answer a complex question and
% a second prompt sequentially answers these sub-questions. In contrast, our approach allows for
% diverse decomposition structures and can use different prompts to answer each sub-question, even
% including symbolic systems. Moreover, rather than generating the entire set of sub-questions (i.e.,
% the decomposition) at once, we can iteratively generate new questions based on the answers to
% previous steps (e.g., our prompt for HotpotQA in Sec. 4.4 is one such use case.)


% \subsection{Chain of Thoughts Reasoning}

% \subsection{Chain of Thoughts Reasoning}

\subsection{Text-to-SQL generation}
\carl{todo}

% Text-to-SQL generation has been studied for decades in both DB and NLP communities. (Warren and Pereira, 1982;
% Zettlemoyer and Collins, 2005; Popescu et al.,
% 2003; Li et al., 2006; Li and Jagadish, 2014; Iyer
% et al., 2017; Zhong et al., 2017; Xu et al., 2017;
% Yu et al., 2018a; Dong and Lapata, 2018; FineganDollak et al., 2018; Guo et al., 2019; Bogin et al., 2019). Majority of works focus on how to fine-tuning model on text-to-sql task. In this paper, we explore how to use LLMs with in-context learning, where the model can only learn with a few examples (demonstration without any fine-tuning). 

==> related_work_v2.tex <==
% \vspace{-0.2pc}

\section{Related Work}

% \vspace{-0.2pc}
% Ron: revised v2
\paragraph{Large Language Models and Prompting.}
%\rc{
As large language models (LLMs) advance \citep{NEURIPS2020_1457c0d6, palm_google}, in-context learning emerged as a new paradigm in natural language processing \citep{prompting_survey}. 
Although LLMs can achieve outstanding performance by prompting them with few-shot examples in context, they struggle with tasks that require complex reasoning. 
As a solution, \citet{wei2022chain} proposed chain-of-thought prompting. 
By explicitly describing intermediate reasoning steps to answer a complex question in the prompts, chain-of-thought prompting improves the accuracy of LLMs by a large margin across many natural language reasoning tasks. 
% \hs{Do we need to say this here: \st{However, chain-of-thought prompting has a key limitation: it often performs poorly on tasks that require generalization of solving problems harder than the demonstration examples, such as compositional generalization} \citep{2022arXiv220510625Z}.}
However, how to apply CoT-style prompting to text-to-SQL remains under-explored. Our work fills the gap by systematically exploring several CoT-style prompting methods for the task.
In particular, we propose a new CoT-style prompting method that guides LLMs to perform reasoning via question decomposition.
We show that text-to-SQL parsing indeed requires multi-step reasoning, and carefully designed CoT-style prompting can help LLMs achieve higher parsing accuracy.
%}
% \vspace{-0.2pc}
\paragraph{Question Decomposition.}
%\rc{
Question decomposition is a method that facilitates QA models by converting a complex problem into a sequence of simpler sub-questions \citep{gupta-lewis-2018-neural, min-etal-2019-multi}.
In light of question decomposition, \citet{2022arXiv220510625Z} proposed least-to-most prompting to solve complex problems with better compositional generalization in two stages. 
The method first prompts LLMs to generate a list of sub-questions as a decomposition of the given problem. 
Then, it uses the sub-questions to guide LLMs to incrementally solve each of them and derive a correct final answer. 
Similarly, our work refers to existing question decomposition methods for text-to-SQL parsing \citep{wolfson-etal-2020-break, DBLP:journals/corr/abs-2112-06311} and designs a novel CoT-style prompting method to improve LLMs' performance.
%Our work is related to \citet{wolfson-etal-2020-break, DBLP:journals/corr/abs-2112-06311}, which applies question decomposition to text-to-SQL parsing, but we explore question decomposition for text-to-SQL parsing under in-context learning context and propose to leverage question decomposition as a novel chain-of-thought style prompting.
We conduct comprehensive experiments and show that our question decomposition prompting outperforms chain-of-thought prompting and least-to-most prompting on several text-to-SQL datasets.
%} 
% \vspace{-0.2pc}
\paragraph{Text-to-SQL Semantic Parsing.} 
%\rc{
Text-to-SQL semantic parsing has long been studied to build natural language interfaces for database applications \citep{data-atis-original, data-geography-original}. 
Since the release of Spider \citep{yu-etal-2018-spider}, a cross-database text-to-SQL benchmark, many parsers have been developed on top of language models to better understand various database schemas \citep{wang-etal-2020-rat, yu2021grappa, deng-etal-2021-structure}.
Recent work starts to explore the potential of LLMs, such as Codex \citep{DBLP:journals/corr/abs-2107-03374}, in text-to-SQL parsing by including database schemas in the prompts \citep{2022arXiv220400498R}, retrieving similar questions as few-shot examples \citep{https://doi.org/10.48550/arxiv.2209.01975}, or reranking SQL parses with their execution results \citep{https://doi.org/10.48550/arxiv.2302.08468}. 
Orthogonal to these methods, our work teaches LLM to perform multi-step reasoning for text-to-SQL parsing without additional engineering efforts.
%or introducing new modules\hs{does the above mentioned \citep{2022arXiv220400498R} introduce new modules? it does not sound so.}.
%Our work is in parallel with these methods and extends this line by teaching LLMs to become a better text-to-SQL parser by itself 
With our question decomposition prompting, an LLM, such as Codex in our experiments, can effectively learn to decompose natural language questions and predict table and column names (Section \ref{sec:promptdesgin}) incrementally in each step with a few in-context examples.
%}

==> tables/QDecomp.tex <==

\begin{table*}[t]
\fontsize{9}{10}\selectfont
% \vspace{1.5 pc}
% \hspace*{-0.4 cm}
\center
\small
\scalebox{1.0}{
\noindent\begin{tabular}{|p{15cm}|}
\hline 
\#\#\# Question: List the problem id and log id which are assigned to the staff named Rylan Homenick.
\\
decompose the question
\\
\\
1. List the problem id and log id.
\\
2. List the problem id and log id which are assigned to the staff.
\\
3. List the problem id and log id which are assigned to the staff named Rylan Homenick.
\\
\\
\# Thus, the answer for the question is: List the problem id and log id which are assigned to the staff named Rylan Homenick.
\texttt{SELECT DISTINCT T2.problem\_id ,  T2.problem\_log\_id FROM staff AS T1 JOIN problem\_log AS T2 ON T1.staff\_id = T2.assigned\_to\_staff\_id WHERE T1.staff\_first\_name = "Rylan" AND T1.staff\_last\_name = "Homenick"}
\\
\hline 
\end{tabular}}
\caption{An example, from the \textbf{QDecomp} promptings on the Spider dataset, demonstrates how this method facilitates the model's ability to break down the original question into simpler sub-questions and generate the final answer directly, without the generation of intermediate SQL queries.}
% \vspace{-1.5 pc}
\label{tb:qdecomp_examples}
\end{table*}

==> tables/QDecomp_table.tex <==

\begin{table*}[t]
\fontsize{9}{10}\selectfont
% \vspace{1.5 pc}
% \hspace*{-0.4 cm}
\center
\small
\noindent\begin{tabular}{|p{15cm}|}
\hline 
\#\#\# Question: List the problem id and log id which are assigned to the staff named Rylan Homenick.
\\
decompose the question
\\
\\
1. List the problem id and log id.
\\
SQL table (column): \hl{problem\_log (problem\_log\_id, problem\_id)}
\\
2. List the problem id and log id which are assigned to the staff.
\\
SQL table (column): \hl{staff (staff\_id)}
\\
3. List the problem id and log id which are assigned to the staff named Rylan Homenick.
\\
SQL table (column): \hl{staff (staff\_first\_name, staff\_last\_name)}
\\
\\
\# Thus, the answer for the question is: List the problem id and log id which are assigned to the staff named Rylan Homenick.
\texttt{SELECT DISTINCT T2.problem\_id ,  T2.problem\_log\_id FROM staff AS T1 JOIN problem\_log AS T2 ON T1.staff\_id = T2.assigned\_to\_staff\_id WHERE T1.staff\_first\_name = "Rylan" AND T1.staff\_last\_name = "Homenick"}
\\
\hline 
\end{tabular}
\caption{A sample prompt taken from the \QDEMPTB promptings on the Spider dataset. Different from the \QDEMP, the model is tasked with identifying intermediate tables and columns, which are highlighted, that match the phrases within the current sub-question.}
% \vspace{-1.5 pc}
\label{tb:qdecomp_intermediate_table}
\end{table*}

==> tables/api_example_prompt.tex <==
\begin{table*}[t]
\fontsize{9}{10}\selectfont
% \vspace{1.5 pc}
% \hspace*{-0.4 cm}
\center
\small
\scalebox{1.0}{
\noindent\begin{tabular}{|p{15cm}|}
\hline 
\#\#\# SQLite SQL tables, with their properties:
\\
\#
\\
\# medicine (id, name, trade\_name, fda\_approved)
\\
\# enzyme (id, name, location, product, chromosome, omim, porphyria)
\\
\# medicine\_enzyme\_interaction (enzyme\_id, medicine\_id, interaction\_type)
\\
\#
\\
\#\#\# What is the total count of enzymes?
\\
SELECT count(*) FROM enzyme
\\
\\
\#\#\# SQLite SQL tables, with their properties:
\\
\#
\\
\# buildings (id, name, city, height, stories, status)
\\
\# companies (id, name, headquarters, industry, sales\_billion, profits\_billion, assets\_billion, market\_value\_billion)
\\
\# office\_locations (building\_id, company\_id, move\_in\_year)
\\
\#
\\
\#\#\# Show the industries shared by companies whose headquarters are "USA" and companies whose headquarters are "China".
\\
SELECT Industry FROM Companies WHERE Headquarters  =  "USA" INTERSECT SELECT Industry FROM Companies WHERE Headquarters  =  "China"
\\
\\

\#\#\# SQLite SQL tables, with their properties:
\\
\#
\\
\# repair (repair\_id, name, launch\_date, notes)
\\
\# machine (machine\_id, making\_year, class, team, machine\_series, value\_points, quality\_rank)
\\
\# technician (technician\_id, name, team, starting\_year, age)
\\
\# repair\_assignment (technician\_id, repair_id, machine_id)
\\
\#
\\
\#\#\# Please show the team that has the most number of technicians.
\\
SELECT Team FROM technician GROUP BY Team ORDER BY COUNT(*) DESC LIMIT 1
\\
\\
\#\#\# SQLite SQL tables, with their properties:
\\
\#
\\
\# allergy\_type (allergy, allergytype)
\\
\# has\_allergy (stuid, allergy)
\\
\# student (stuid, lname, fname, age, sex, major, advisor, city\_code)
\\
\#
\\
\#\#\#  What are the allergies and their types that the student with first name Lisa has? And order the result by name of allergies.
\\
SELECT T1.Allergy ,  T1.AllergyType FROM Allergy\_type AS T1 JOIN Has\_allergy AS T2 ON T1.Allergy  =  T2.Allergy JOIN Student AS T3 ON T3.StuID  =  T2.StuID WHERE T3.Fname  =  "Lisa" ORDER BY T1.Allergy
\\
\\
\#\#\# SQLite SQL tables, with their properties:
\\
\#
\\
\# stadium (stadium\_id, location, name, capacity, highest, lowest, average)
\\
\# singer (singer\_id, name, country, song\_name, song\_release\_year, age, is\_male)
\\
\# concert (concert\_id, concert\_name, theme, stadium\_id, year)
\\
\# singer\_in\_concert (concert\_id, singer\_id)
\\
\#
\\
\#\#\# How many singers do we have?
\\
\hline 
\end{tabular}}
\caption{An example taken from the standard promptings for \textbf{4-shot} on the Spider dataset.}
% \vspace{-1.5 pc}
\label{tb:app_ex_standard}
\end{table*}



\begin{table*}[t]
\fontsize{9}{10}\selectfont
% \vspace{1.5 pc}
% \hspace*{-0.4 cm}
\center
\small
\scalebox{1.0}{
\noindent\begin{tabular}{|p{15cm}|}
\hline 
\#\#\# SQLite SQL tables, with their properties:
\\
\#
\\
\# inst (instid, name, country)
\\
\# authors (authid, lname, fname)
\\
\# papers (paperid, title)
\\
\# authorship (authid, instid, paperid, authorder)
\\
\#
\\
\#\#\# Find papers whose second author has last name "Turon" and is affiliated with an institution in the country "USA".
\\
\# Let's think step by step
\\
\\
\# This query chooses records from the papers table, followed by joining the authorship table on the paperid column. It then filters for rows where the authorder is 2 and the lname is 'Turon', joining the authors table on the authid column. It then filters for rows where the country is 'USA', joining the inst table on the instid column. It then selects the title column.
\\
\\
\# Thus, the answer for the question is: Find papers whose second author has last name "Turon" and is affiliated with an institution in the country "USA".
SELECT t3.title FROM authors AS t1 JOIN authorship AS t2 ON t1.authid  =  t2.authid JOIN papers AS t3 ON t2.paperid  =  t3.paperid JOIN inst AS t4 ON t2.instid  =  t4.instid WHERE t4.country  =  "USA" AND t2.authorder  =  2 AND t1.lname  =  "Turon"
\\
\\
\#\#\# SQLite SQL tables, with their properties:
\\
\#
\\
\# staff (staff\_id, gender, first\_name, last\_name, email\_address, phone\_number)
\\
\# customers (customer\_id, customer\_type\_code, address\_line\_1, address\_line\_2, town\_city, state, email\_address, phone\_number)
\\
\# products (product\_id, parent\_product\_id, product\_category\_code, date\_product\_first\_available, date\_product\_discontinued, product\_name, product\_description, product\_price)
\\
\# complaints (complaint\_id, product\_id, customer\_id, complaint\_outcome\_code, complaint\_status\_code, complaint\_type\_code, date\_complaint\_raised, date\_complaint\_closed, staff\_id)
\\
\#
\\
\#\#\# List the name of all products along with the number of complaints that they have received.
\\
\# Let's think step by step
\\
\# This query chooses records from the products table, followed by joining the complaints table on the product\_id column. It then groups the results by product\_name, followed by selecting the product\_name column and the count of each product\_name.
\\
\# Thus, the answer for the question is: List the name of all products along with the number of complaints that they have received.
SELECT t1.product\_name ,  count(*) FROM products AS t1 JOIN complaints AS t2 ON t1.product\_id  =  t2.product\_id GROUP BY t1.product\_name

\\

\\
\#\#\# SQLite SQL tables, with their properties:
\\

\#
\\
\# workshop (workshop\_id, date, venue, name)
\\
\# submission (submission\_id, scores, author, college)
\\
\# acceptance (submission\_id, workshop\_id, result)
\\
\#
\\
\\
\#\#\# For each submission, show the author and their affiliated college.
\\
\# Let's think step by step
\\
\# This query chooses records from the submission table. It then selects the author and college columns.
\\
\# Thus, the answer for the question is: For each submission, show the author and their affiliated college.
SELECT Author ,  College FROM submission
\\
\\
\#\#\# SQLite SQL tables, with their properties:
\\
\#
\\
\# buildings (id, name, city, height, stories, status)
\\
\# companies (id, name, headquarters, industry, sales\_billion, profits\_billion, assets\_billion, market\_value\_billion)
\\
\# office\_locations (building\_id, company\_id, move\_in\_year)
\\
\#
\\
\\
\#\#\# Show the industries shared by companies whose headquarters are "USA" and companies whose headquarters are "China".
\\

\# Let's think step by step

\\

\# This query chooses records from the companies table, followed by a WHERE clause that selects records where the headquarters column is equal to USA. It then selects the industry column.
\\

\# The second query chooses records from the companies table, followed by a WHERE clause that selects records where the headquarters column is equal to China. It then selects the industry column. The INTERSECT clause returns the intersection of the two queries.

\\

\# Thus, the answer for the question is: Show the industries shared by companies whose headquarters are "USA" and companies whose headquarters are "China".
SELECT Industry FROM Companies WHERE Headquarters  =  "USA" INTERSECT SELECT Industry FROM Companies WHERE Headquarters  =  "China"
\\
\\
\#\#\# SQLite SQL tables, with their properties:
\\
\#
\\
\# stadium (stadium\_id, location, name, capacity, highest, lowest, average)
\\
\# singer (singer\_id, name, country, song\_name, song\_release\_year, age, is\_male)
\\
\# concert (concert\_id, concert\_name, theme, stadium\_id, year)
\\
\# singer\_in\_concert (concert\_id, singer\_id)
\\
\#
\\
\\
\#\#\# How many singers do we have?
\\
\hline 
\end{tabular}}
\caption{An example taken from the \COT promptings for \textbf{4-shot} on the Spider dataset.}
% \vspace{-1.5 pc}
\label{tb:app_api_ex_chain_of_thought}
\end{table*}

==> tables/app_error_analysis.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{lcccc}
\toprule 
& Semantic & Ambiguous & \multirow{2}{*}{Invalid SQL}
\\
& Incorrect & Correct & 
\\
\midrule
% QDecomp  & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{}  \\ 
% + InterCOL \\
% (4-shots)\\
% \midrule 
QDecomp  & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{}  \\ 
+ InterCOL & 19 & 7 & 4 \\
(8-shots)\\ 
\midrule 
\end{tabular}
\caption{Error analysis of \QDEMPTB prompting on 30 random problems, where we analyze the results obtained from the 8-shots setting. These errors were categorized that semantic incorrect, ambiguous correct, and invalid SQL query.}
\label{tb:app_error_analysis}
\end{table}


==> tables/chain_of_thought_error.tex <==

\begin{table*}[t]
\fontsize{9}{10}\selectfont
\center
\small
\scalebox{1.0}{
\noindent\begin{tabular}{p{1.3cm}p{13.5cm}}
\hline 
& \textbf{Semantic Incorrect}
\\
Question & How many United Airlines flights go to City 'Aberdeen'?
\\
\hline 
\textbf{\COT} & \# This query chooses records from the flights table, \colorbox{pink}{followed by joining the airlines table on the airline} \colorbox{pink}{column. It then filters the results where the airline column is United Airlines and the destairport column} \colorbox{pink}{is Aberdeen.} It then selects the count of the records.
\\
& \# Thus, the answer for the question is: How many United Airlines flights go to City 'Aberdeen'?
\texttt{SELECT count(*) FROM flights AS T1 JOIN airlines AS T2 \colorbox{pink}{ON T1.airline}  \colorbox{pink}{=  T2.airline WHERE T2.airline  = 'United Airlines' AND T1.destairport  =} \colorbox{pink}{  'Aberdeen'}}
\\
\\
\textbf{Least-to-} & Q: How many United Airlines flights go to City?
\\
\textbf{Most} & A:\texttt{SELECT count(*) FROM flights \colorbox{pink}{WHERE airline  =  'United Airlines' AND} \colorbox{pink}{destairport  =  'City'}}
\\
 & Q: How many United Airlines flights go to City 'Aberdeen'?
\\
 & A:\texttt{SELECT count(*) FROM flights \colorbox{pink}{WHERE airline  =  'United Airlines' AND} \colorbox{pink}{destairport  =  'Aberdeen'}}
\\
Gold & \texttt{SELECT count(*) FROM flights AS T1 JOIN 
 airports AS T2 ON T1.destairport  =  T2.airportcode JOIN airlines AS T3 ON T3.uid  =  T1.airline WHERE T2.city  =  'Aberdeen' AND T3.airline  =  'United Airlines'}
\\
\midrule
& \textbf{Ambiguous Correct}
\\
Question & What are the details for the paragraph that includes the text 'Korea'
\\
\hline 
\textbf{\COT} & \# This query chooses records from the Paragraphs table, followed by a WHERE clause that selects records 
where the paragraph\_text column contains the word Korea. \colorbox{pink}{It then selects the paragraph\_id, document\_id,} \colorbox{pink}{and paragraph\_text columns.}


\\
& \# Thus, the answer for the question is: What are the details for the paragraph that includes the text 'Korea’ ? \texttt{\colorbox{pink}{SELECT paragraph\_id, document\_id, paragraph\_text} FROM paragraphs WHERE paragraph\_text LIKE  'Korea'}
\\
Gold & \texttt{SELECT other\_details from paragraphs where paragraph\_text like 'Korea'}
\\
\hline 
\end{tabular}}
\caption{Examples of error types, as made by the Codex with \COT and \LTM promptings.\hs{there are many issues in this figure. see some comments in Figure 1. Caption needs to be rephrased as well.}}
\label{tb:chain_of_thought_error_types}
\end{table*}

% BOTH LEAST-TO-MOST AND CHAIN-OF-THOUGHT FAILED


% \begin{table*}[t]
% \fontsize{9}{10}\selectfont
% \center
% \small
% \scalebox{1.0}{
% \noindent\begin{tabular}{p{1.3cm}p{13.5cm}}
% \hline 
% & \textbf{Semantic Incorrect}
% \\
% Question & Show the name and the release year of the song by the youngest singer.
% \\
% \hline 
% \textbf{\COT} & \# This query chooses records from the singer table, \colorbox{pink}{followed by joining the singer\_in\_concert table on the} \colorbox{pink}{singer\_id column. It then joins the concert table on the concert\_id column.} It then orders the results by the age column in ascending order. The LIMIT 1 clause returns only the first row of the result set. It then selects the song\_name and song\_release\_year columns. 
% \\
% & \# Thus, the answer for the question is: Show the name and the release year of the song by the youngest singer. \texttt{SELECT T1.song\_name, T1.song\_release\_year FROM singer AS T1 \colorbox{pink}{JOIN singer\_in\_concert AS T2 ON T1.singer\_id  =  T2.singer\_id JOIN } \colorbox{pink}{concert AS T3 ON T2.concert\_id  =  T3.concert\_id} ORDER BY T1.age LIMIT 1}
% \\
% \\
% \textbf{Least-to-} & Q: Show the name and the release year of the song.
% \\
% \textbf{Most} & A: \texttt{SELECT song\_name, song\_release\_year FROM singer}
% \\
% \\
%  & Q: Show the name and the release year of the song by the youngest singer.
% \\
%  & A:\texttt{SELECT T1.song\_name,  T1.song\_release\_year FROM singer AS T1 \colorbox{pink}{JOIN  } \colorbox{pink}{singer\_in\_concert AS T2 ON T1.singer\_id  =  T2.singer\_id JOIN concert  }
%  \colorbox{pink}{AS T3 ON T2.concert\_id  =  T3.concert\_id} ORDER BY T1.age DESC LIMIT 1}
% \\
% Gold & \texttt{SELECT song\_name, song\_release\_year FROM singer ORDER BY age LIMIT 1}
% \\
% \midrule
% & \textbf{Ambiguous Correct}
% \\
% Question & What are the details for the paragraph that includes the text 'Korea'
% \\
% \hline 
% \textbf{\COT} & \# This query chooses records from the Paragraphs table, followed by a WHERE clause that selects records 
% where the paragraph\_text column contains the word Korea. \colorbox{pink}{It then selects the paragraph\_id, document\_id,} \colorbox{pink}{and paragraph\_text columns.}


% \\
% & \# Thus, the answer for the question is: What are the details for the paragraph that includes the text 'Korea’ ? \texttt{\colorbox{pink}{SELECT paragraph\_id, document\_id, paragraph\_text} FROM Paragraphs WHERE paragraph\_text LIKE  'Korea'}
% \\
% Gold & \texttt{SELECT other\_details from paragraphs where paragraph\_text like 'Korea'}
% \\
% \hline 
% \end{tabular}}
% \caption{Examples of error types, as made by Codex with \COT promptings.\hs{there are many issues in this figure. see some comments in Figure 1. Caption needs to be rephrased as well.} \carl{shorter example}}
% \label{tb:chain\_of\_thought\_error\_types}
% \end{table*}

% % BOTH LEAST-TO-MOST AND CHAIN-OF-THOUGHT FAILED

==> tables/chainofthoughtprompt.tex <==

\begin{table*}[t]
\fontsize{9}{10}\selectfont
% \vspace{1.5 pc}
% \hspace*{-0.4 cm}
\center
\small
\scalebox{1.0}{
\noindent\begin{tabular}{|p{15cm}|}
\hline 
\#\#\# Find papers whose second author has last name "Turon" and is affiliated with an institution in the country "USA".
\\
\# Let's think step by step
\\
\\
This query chooses records from the papers table, followed by joining the authorship table on the paperid column. It then filters for rows where the authorder is 2 and the lname is 'Turon', joining the authors table on the authid column. It then filters for rows where the country is 'USA', joining the inst table on the instid column. It then selects the title column.
\\
\\
\# Thus, the answer for the question is: Find papers whose second author has last name "Turon" and is affiliated with an institution in the country "USA".
\\
\\
\texttt{SELECT t3.title FROM authors AS t1 JOIN authorship AS t2 ON t1.authid  =  t2.authid JOIN papers AS t3 ON t2.paperid  =  t3.paperid JOIN inst AS t4 ON t2.instid  =  t4.instid WHERE t4.country  =  "USA" AND t2.authorder  =  2 AND t1.lname  =  "Turon"}
\\
\hline 
\end{tabular}}
\caption{An example taken from the \COT promptings on the Spider dataset. \hs{do we still need an example here, give Figure 1?}}
% \vspace{-1.5 pc}
\label{tb:chain_of_thought}
\end{table*}

==> tables/error_analysis.tex <==
\begin{table}[h]
\centering
\small
\scalebox{0.95}{\begin{tabular}{lcccc}
\toprule 
& Semantic & Ambiguous & \multirow{2}{*}{Invalid SQL}
\\
& Incorrect & Correct & 
\\
\midrule
\COT & 38 & 3 & 9  \\ \midrule 
\LTM & 17 & 3 & 7  \\ \midrule 
QDecomp  & \multirow{2}{*}{13} & \multirow{2}{*}{2} & \multirow{2}{*}{3}  \\ 
+ InterCOL \\
\midrule 
\end{tabular}}
\caption{Error analysis of 50 questions that are answered incorrectly by the model with \COT prompting. The errors are classified into three types: semantic incorrect, ambiguous correct, and invalid SQL.}
\label{tb:error_analysis}
\end{table}


==> tables/evaluation_g3.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lcc}
\toprule
& Random & G3 \\ \midrule 
Standard & 63.2 $\pm$ 2.51 & 58.7 $\pm$ 3.32 \\ 
Least-to-Most & 66.0 $\pm$ 2.48 & 63.3 $\pm$ 1.95 \\ \midrule 
QDecomp & \underline{67.4} $\pm$ 1.89 & \underline{66.5} $\pm$ 0.63 \\ 
+ InterCOL & \textbf{68.4} $\pm$ 2.05 & \textbf{68.8} $\pm$ 1.16 \\ 
\bottomrule
\end{tabular}
\caption{
8-shot test-suite accuracy of Codex on Spider Dev using different prompting methods and API Doc format with \textbf{G3 in-context examples}. We also include the overall standard execution accuracy (EX) in parenthesis for reference.
}
\vspace{-1pc}
\label{tab:spider_result_g3}
\end{table}

==> tables/least_to_most.tex <==
\begin{table*}[t]
\fontsize{9}{10}\selectfont
% \vspace{1.5 pc}
% \hspace*{-0.4 cm}
\center
\small
\scalebox{1.0}{
\noindent\begin{tabular}{|p{15cm}|}
\hline 
% Q: "Which apartments have unit status availability of both 0 and 1? Return their apartment numbers."
% A: To answer the above question, we need to know: "Return their apartment numbers.", "Return their apartment numbers. Which apartments have unit status availability of 0?".
% \\
% \\
\multirow{2}{*}{\LTM prompting (question decomposition stage)} 
\\ 
\\
\hline
Q: "Find the name of customers who have loans of both Mortgages and Auto."
A: To answer the above question, we need to know: "Find the name of customers", "Find the name of customers who have loans", "Find the name of customers who have loans of Mortgages".
\\
\\
Q: “What are the names of the stations which serve Ananthapuri Express trains?”
\\
A: To answer the above question, we need to know: "What are the names of the stations?", "What are the names of the stations which serve "Ananthapuri Express" trains?".
\\
\hline
\multirow{2}{*}{\LTM prompting (question solving stage)}
\\
\\
\hline
Q: “What are the names of the stations?”
\\
A:~\texttt{SELECT name FROM station}
\\
\\
Q: “What are the names of the stations which serve Ananthapuri Express trains?”
\\
A:~\texttt{SELECT T2.name FROM train\_station AS T1 JOIN station AS T2 ON T1.station\_id  = T2.station\_id JOIN train AS T3 ON T3.train\_id  =  T1.train\_id WHERE T3.Name  = Ananthapuri Express}
\\
\\
Q: “What are the names of the stations which serve both Ananthapuri Express and Guruvayur Express trains?”
\\
A:~\texttt{SELECT T2.name FROM train\_station AS T1 JOIN station AS T2 ON T1.station\_id  =  T2.station\_id JOIN train AS T3 ON T3.train\_id  =  T1.train\_id WHERE T3.Name  =  Ananthapuri Express AND T3.Name  =  Guruvayur Express}
\\
\hline
\end{tabular}}
\caption{Question decomposition stage (upper column) and solving stage (lower column) of \LTM prompting for a problem on the Spider dataset.\hs{caption is very confusing.} \carl{updated}}
% \vspace{-1.5 pc}
\label{tb:least_to_most_promoting}
\end{table*}


% \begin{table*}[t]
% \fontsize{9}{10}\selectfont
% % \vspace{1.5 pc}
% % \hspace*{-0.4 cm}
% \center
% \small
% \scalebox{1.0}{
% \noindent\begin{tabular}{|p{15cm}|}
% \hline 
% Q: “What are the names of the stations?”
% \\
% A:~\texttt{SELECT name FROM station}
% \\
% \\
% Q: “What are the names of the stations which serve Ananthapuri Express trains?”
% \\
% A:~\texttt{SELECT T2.name FROM train\_station AS T1 JOIN station AS T2 ON T1.station\_id  = T2.station\_id JOIN train AS T3 ON T3.train\_id  =  T1.train\_id WHERE T3.Name  = Ananthapuri Express}
% \\
% \\
% Q: “What are the names of the stations which serve both Ananthapuri Express and Guruvayur Express trains?”
% \\
% A:~\texttt{SELECT T2.name FROM train\_station AS T1 JOIN station AS T2 ON T1.station\_id  =  T2.station\_id JOIN train AS T3 ON T3.train\_id  =  T1.train\_id WHERE T3.Name  =  Ananthapuri Express AND T3.Name  =  Guruvayur Express}
% \\
% \hline 
% \end{tabular}}
% \caption{An example taken from the \LTM promptings (solving) on the Spider dataset.}
% % \vspace{-1.5 pc}
% \label{tb:least_to_most}
% \end{table*}
